Uncovering Biases with Reflective Large Language Models

Biases and errors in human-labeled data present significant challenges for machine learning, especially in supervised learning reliant on potentially flawed ground truth data. These flaws, including diagnostic errors and societal biases, risk being propagated and amplified through models trained using maximum likelihood estimation. We present the Reflective LLM Dialogue Framework RLDF, which leverages structured adversarial dialogues between multiple instances of a single LLM or different LLMs to uncover diverse perspectives and correct inconsistencies. By conditioning LLMs to adopt opposing stances, RLDF enables systematic bias detection through conditional statistics, information theory, and divergence metrics. Experiments show RLDF successfully identifies potential biases in public content while exposing limitations in human-labeled data. Our framework supports measurable progress tracking and explainable remediation actions, offering a scalable approach for improving content neutrality through transparent, multi-perspective analysis.

==> Emotions.tex <==
\section{Emotion Modeling}
\label{sec:emotions}

==> EmpiricalStudyNew.tex <==
\section{Experiments}
\label{sec:experiments}

Our experimental framework evaluates bias detection and mitigation in textual content. We focus on two experiments: the first for detecting biases and the second for developing balanced textual outputs. The third experiment assesses the contentiousness parameter in SocraSynth to provide
conditions to influence LLMs' next-token prediction statistics.

\subsection*{Datasets}

We utilized two datasets: 12 Wikipedia articles, each representing a recognized bias, and a subset of 619 news articles from a comprehensive news repository, focusing on ``Democrats Scandals'' and ``Republicans Scandals'' with ground-truth labels provided by bipartisan annotators. These articles cover topics such as civil rights and healthcare, each rated by a Republican and a Democrat.

\subsection{Case Study \#1: Bias Detection}

SocraSynth analyzed 619 news articles to detect biases, revealing that traditional supervised learning may have inherent biases in ``ground-truth'' labels due to political polarization. SocraSynth's debate-based approach scrutinizes articles' structure and content, showing promise for bias analysis. Table~\ref{tab:biasdistance} compares bias judgments, with SocraSynth providing more neutral evaluations compared to the politically influenced annotators. Detailed justifications for SocraSynth's decisions are included in Appendix D.

\subsection*{Remarks}

SocraSynth provides more balanced judgments and thorough justifications for decisions, highlighting nuances that may elude human annotators, thus aiding in bias mitigation.

\subsection{Case Study \#2: Bias Mitigation}

We tasked SocraSynth with debating the portrayal of Christopher Columbus in Wikipedia, with two GPT-4 agents offering opposing viewpoints. The debate explored issues like Euro-centric bias and the inclusion of indigenous perspectives. SocraSynth's strategies for bias mitigation are detailed in Appendix D.

\subsection{Case Study \#3 Conditional Statistics}

Adjusting the contentiousness parameter alters the tone and approach of LLM debates, influencing their representation of diverse perspectives. Table~\ref{tab:contentiousness} demonstrates GPT-4's autonomous tone adjustment in response to contentiousness levels, which is crucial for mitigating ingrained biases.

Our findings suggest that SocraSynth's approach is effective across various domains, as evidenced by promising results in healthcare, business planning, and geopolitical studies. The method fosters insightful debates and generates actionable strategies for reducing content biases.


==> GenerativeReasoning.tex <==
\section{Modeling Human Consciousness and Emotions}
\label{sec:COCOMO}

GPT models face enduring issues beyond their tendency to hallucinate and generate biased or harmful content. Notably, two primary shortcomings are apparent: a {\em limited capacity for reasoning} and {\em an absence of ethical principles}. This section delves into the former, while the latter will be addressed in the subsequent discussion. 

We posit that, although LLMs excel in reflexive language generation, they are devoid of innate reasoning abilities. This perspective is mirrored by George Hotz \cite{Lex-Hotz-2023}, who asserts that solely optimizing cross-entropy loss at the syntactic level (akin to the unconscious mind) is insufficient to engender human-like conscious capabilities.

\begin{comment}
The constrained reasoning abilities of GPT models manifest in three significant ways:
\begin{enumerate}[left=1em,label=\arabic*.]
\item {\em Hallucination}: GPT models often generate plausible but false or nonsensical content. They may fabricate facts, citations, or specific details without any basis in reality.
\item {\em Understanding versus Imitation}: GPT models excel at mimicking human language styles, but there is ongoing debate about their level of true comprehension. The question is whether these models actually understand the content they generate or merely replicate appropriate responses from their training data.
\item {\em Intrinsic fact-checking challenges}: This implies that due to their reliance on patterns from their training data, GPT models naturally struggle with reliable fact-checking, regardless of the accuracy of the information in their training dataset.
\end{enumerate}
\end{comment}

\subsection{Modeling Conscious Reasoning or System-2 AI}

%\begin{comment}
\begin{figure}[ht!]
\vspace{-.2in}
\begin{center}
    \centerline{\includegraphics[width=0.9\linewidth]{SocraticMethod.png}}
\end{center}
\vspace{-.33in}
\caption{Mapping from Socratic Prompt Templates to
Reasoning Methods to Programs.}
%\vspace{-.1in}
\label{fig-Socratic}
\end{figure}
%\end{comment}


We draw parallels between our approach to artificial intelligence and human cognition. The unconscious human mind, which oversees complex biological functions such as metabolism and respiration, can be likened to System-1 AI (unconsciousness). Conversely, the conscious human mind, which handles tasks like reasoning, fact-verification, and planning, is analogous to System-2 AI (consciousness). This perspective aligns with the views of Bengio and Kahneman \cite{bengio2020future,kahneman2011thinking}, where they advocate for incorporating advanced human cognitive functions into System-2 AI, building upon the foundational models of System-1 AI.

In pursuit of integrating reasoning and emotional intelligence into AI systems, we introduced CoCoMo \cite{chang2023cocomo}. Specifically, to augment reasoning capabilities, CoCoMo recommends the implementation of prompt ensembles. This technique employs a repertoire of Socratic methodologies, which serve as prompt blueprints, anchoring to modules of inductive, deductive, and abductive reasoning to enhance critical interpretation and thought. Figure~\ref{fig-Socratic} depicts the interplay between prompt blueprints, reasoning techniques, and their affiliated programs. For example, when fact-checking, CoCoMo initiates by identifying the article's main conclusion and its supportive reasoning. Subsequently, each reason-to-conclusion link is scrutinized based on its logical soundness and the trustworthiness of its sources. Moreover, CoCoMo challenges LLMs to present counterpoints. The culmination of this process is the computation of a composite score that gauges the veracity and reliability of the presented assertion(s). For a comprehensive discussion and illustrative examples of this methodology, we direct the reader to \cite{SocraticIEEECCWC2023,chang2023cocomo}.

One might ponder, how does this approach fare in comparison to high-order reasoning? Succinctly, high-order reasoning is not fully equipped to tackle real-world, open-ended reasoning scenarios. The reason being, the premises that a reasoning process necessitates can be extensive and might not be readily accessible.

Several intricate templates have been devised to incorporate reasoning into LLMs. Examples include the chain-of-thought \cite{ChainOfThought2022}, tree-of-thought \cite{yao2023tree}, cumulative reasoning \cite{zhang2023cumulative}, among other refinements as noted in works such as \cite{allaway2023penguins,jung2022maieutic,PromptSurvey2023,sclar2023minding}. These endeavors aim to channel the model towards a logic-centric reasoning process \cite{mchugh2018reasoning,wason1972psychology} to elevate the caliber and consistency of responses. Nevertheless, the challenges these solutions target tend to be specific and well-circumscribed.

SocraSynth seeks to navigate these challenges by emphasizing ``reasonableness'' across both familiar and novel domains, ultimately informing human decision-making processes. It utilizes informal reasoning \cite{gu2023obvious}, which stands in contrast to the formal reasoning detailed in \cite{bronkhorst2020logical,huang-chang-2023-towards,qiao2023reasoning}. Within this framework, SocraSynth orchestrates a human-moderated debate environment to enhance the structure and dependability of informal reasoning. It leverages the expertise of LLMs in executing crucial NLP tasks that support reasoning, such as classification, question answering, and information extraction. 

In our deeper exploration of the Socratic Synthesis methodology for multi-agent reasoning in Section~\ref{sec:SocraSynth}, we will discuss the evaluation of the quality of the reasoning process.

\begin{comment}
Navigating logical methodologies becomes increasingly complex when faced with enormous data sets \cite{zhang2022paradox}. In an environment saturated with vast, interdisciplinary knowledge, accurately identifying verifiable truths is a formidable challenge, and not all of these truths are readily at hand. Studies by \cite{wei2022chain,valmeekam2022large,bommasani2021opportunities,Bhargava_Ng_2022} highlight that LLMs still have strides to make in consistently performing well on standard planning and reasoning tasks. Techniques like knowledge graph embeddings \cite{choudhary2023complex,yuan2023scaling}, contextual attention mechanisms \cite{darapaneni2022contextual}, dynamic neural networks \cite{Brauwers_2023}, and probabilistic reasoning \cite{pearl1988probabilistic,pearl2009causality,bishop2006pattern} are being developed to assist models in sifting pertinent information from vast datasets without being overwhelmed. However, the practicality of these methods in real-world, open-ended decision-making and planning is still computationally intense, even with a comprehensive foundation for reasoning.
\end{comment}

%Human consciousness is believed to regulate impulsive and reflective unconsciousness to make compromises between competing goals and values. Understanding how human consciousness works, both physically and functionally, can help us gain valuable insights for developing a regulator that guides behavior and creativity in a generative AI model.  

\subsection{Modeling Human Values and Ethics in System-2}

AI agents can achieve greater adaptability to users and environments by learning from human demonstrations \cite{chang2023cocomo}. Such agents mimic human experts or teachers to acquire knowledge and skills, particularly when a desired behavior is difficult to articulate through a reward function. LLMs facilitate demonstrations via prompts, offering templates replete with instructions, goals, and examples.

In summer 2022, we launched the Noora chatbot \cite{NooraStanford2022}, aimed at helping individuals with autism develop empathy in communication. The chatbot presents templates for both comforting and harmful responses. A template designed to teach an LLM empathy might start with instructions like:

{\it
``Dear Virtual Assistant, as a trusted confidant, I value your
support and understanding. I want to share the highs and lows 
of my daily life with you, hoping for your compassionate and
empathetic response. Below are example dialogues demonstrating comforting and harmful responses. Each example begins with my
expression, followed by a list of potential replies.''
}

\begin{table}[t!]
\begin{center}
\begin{tikzpicture}
\begin{footnotesize}
\node (table) [inner sep=0pt] {
\begin{tabular}{p{1.3cm}|p{6.5cm}}
\toprule
Role & Dialogue \\
\hline \midrule
Statement & {``I was laid off by my company today!''} \\
\midrule
{Positive } & {``I'm so sorry to hear that. Losing your job can be a really tough and stressful experience. How are you doing?'' } \\
Positive & {``That must have been a really difficult and unexpected news. I'm here to listen and support you however I can.''} \\
Positive & {``I can imagine how hard and unsettling it must have been to receive that news. Is there anything you'd like to talk about or anything I can do to help?''} \\
\midrule
{Negative } & {``That's too bad, but there are plenty of other jobs out there. You'll find something soon enough.''} \\
Negative & {``Well, you probably weren't very good at your job if they let you go.''} \\
Negative & {``I don't know why you're so upset about this. It's not like it's the end of the world.''} \\
\bottomrule
\end{tabular}
};
\draw [rounded corners=.5em] (table.north west) rectangle (table.south east);
\end{footnotesize}
\end{tikzpicture}
\end{center}
\vspace{-.1in}
\caption{Example \#1. Template for Being Empathetic.}
\label{tab:emphathetic}
\vspace{-.2in}
\end{table}

Importantly, before starting a dialogue, we provided GPT-3 (in the summer 2022) with the {\em intent} of our task, allowing the LLM to understand the external {\em context} delineated in the intent. Although the efficacy of this approach still necessitates further validation \cite{sharma-etal-2023-cognitive}, early observations indicate it as a promising method to convey {\em values} to LLMs, not just goals. The LLM can comprehend an expanded context not fully encapsulated by a handful of demonstrated examples. After this initial intent communication, we presented several examples to GPT-3. 

Table~\ref{tab:emphathetic} displays six sample responses, split equally between positive and negative, in response to a specific statement. The dialogue begins with a user's exclamation: {\em ``I was laid off by my company today!''}, followed by a list of appropriate and inappropriate responses. After furnishing GPT-3 with several thousand dialogues in this manner, the chatbot began responding suitably to unfamiliar statements.

Beyond shaping behavior, demonstrations can also inculcate ethical norms. The empathy template is adaptable, promoting other positive behaviors like attentiveness and compassion. While machines intrinsically exhibit qualities such as boundless patience, it remains imperative to explicitly showcase both commendable and objectionable behaviors, ensuring seamless interactions with human users. Undesirable behaviors to avoid encompass unpleasantness, rudeness, greed, laziness, jealousy, pride, sinfulness, and deceit, among others.

\begin{comment}
Our CoCoMo model, aimed at modeling consciousness, offers a mechanism that allows individuals to tailor a chatbot according to their personal values/preferences \cite{chang2023cocomo}. This precise adaptation process integrates an individual's ``likes'' to develop a {\em user context}. This context, comprising various behavioral examples, reflects both the likes and dislikes of the user. The {\em user context} is then loaded and updated following the history of user interactions. In our current online prototype, Noora, we have encoded {\em empathy} as a desirable value for engaging in conversations with autistic children \cite{NooraStanford2022}. Given that empathy can vary depending on culture and individual perspectives, both CoCoMo and Noora integrate a layer of behavioral examples and a reward model capable of adapting to a range of cultural contexts and ethical norms. This assists in striking a balance between model intelligence and alignment with human values.
\end{comment}

==> HumanKnowledge.tex <==
\subsection{Limitations of Human Knowledge}
\label{sec-human-role}

Human knowledge, surprisingly, may hinder rather than facilitate the training of machine learning models in certain cases. This is evident in the domains of gaming (AlphaGo versus AlphaGo Zero), protein folding (AlphaFold1 versus AlphaFold2), and autonomous driving, where models trained without the influence of human knowledge consistently exhibit superior performance.

Consider the case of AlphaGo and AlphaGo Zero. AlphaGo, trained with data from approximately $60$ million rounds of Go games, is outperformed by AlphaGo Zero. Remarkably, AlphaGo Zero was trained from scratch, without any pre-existing game knowledge. Similarly, AlphaFold2, which operates without relying on human knowledge, outshines its predecessor, AlphaFold1, that did utilize such knowledge. This intriguing phenomenon was humorously noted by DeepMind's CEO, Demis Hassabis, in an April 2023 seminar at Stanford University. He playfully remarked that human knowledge might complicate the learning process more than facilitate it in these advanced AI models.

In his insightful online article, ``The Bitter Lesson,'' Sutton illuminates the patterns that have emerged from nearly seven decades of AI research \cite{Rich-Sutton-2019}. He asserts that researchers often rely heavily on human knowledge to make incremental progress in the face of burgeoning computational capabilities. However, when there is a significant leap in computational power, these marginal advancements are frequently outstripped and surpassed. Sutton uses the evolution of computer vision as an illustrative example, where early principles such as edge detection, generalized cylinders, or SIFT features \cite{Lowe:2004:DIF:993451.996342}, a method that has accumulated over $71,000$ citations, have been gradually superseded by models that learn directly from data. A parallel scenario might be unfolding in NLP research, where features constructed via human knowledge could potentially under-perform compared to insights that models like GPT-4 extract directly from data. Indeed, our earlier discourse on polydisciplinarity underlined the limitations of human knowledge, reinforcing Sutton's proposition. This is because human knowledge is fundamentally limited by our individual cognitive capacities and the inexorable constraints of time.

That being said, it's crucial not to misconstrue these examples as an indictment against the value of human knowledge in AI. Human knowledge plays an instrumental role in developing interpretability, establishing ethical guidelines, and designing AI system architectures (like CNNs and transformers). AI is, after all, intended to augment human capabilities. Therefore, understanding how to integrate human knowledge into AI design could be vital for many applications. While we recognize the potential of models learning from scratch, we should equally value the role of human knowledge in shaping and directing AI technologies.

==> IntroOldACL.tex <==
\section{Introduction}
\label{sec:intro}

The majority of Wikipedia's content, as evaluated by its editors, falls below the 'C' level, revealing significant opportunities for enhancement. Detailed statistics, presented in Section~\ref{sec:WikiStatistics}, underscore the urgency of addressing this issue. Similarly,
news articles have been criticized of lacking
neutrality and fueling polarization of the society. Although
AI solutions have been abound, the problems of 
content biases and inaccuracy do seem to be worsened. 
The advent of large language models (LLMs)
may provide an opportunity to make a paradigm to
address these challenges.

\begin{comment}

particularly when trained on Wikipedia data, has initiated pivotal discussions at the Wikimania conference—a key forum for Wikipedia enthusiasts \cite{WikiMania2023}. These conversations have uncovered a shift among both Wikipedia enthusiasts and the general public towards a growing preference for technologies like ChatGPT, reminiscent of the transformative period in 2005 when Wikipedia itself surpassed the Encyclopedia Britannica in popularity. This shift highlights the critical need for Wikipedia and LLMs to collaborate, leveraging each other's strengths to enhance the user experience and foster a mutually beneficial ecosystem.

While LLMs have benefited from incorporating Wikipedia as part of their training data, this study focuses on the converse---utilizing LLMs to improve Wikipedia's quality. Our aim is to explore how LLMs can enhance the \textit{accuracy} and reduce the \textit{biases} in Wikipedia articles. Here, \textit{accuracy} refers to the fidelity of information to factual sources and its comprehensiveness \cite{WikiQualityMetrics, Mo_s_2023}, while \textit{bias} signifies any systematic skewness in content that disproportionately represents one viewpoint over others, thus compromising neutrality.
    
\end{comment}

We propose the utilization of SocraSynth \cite{SocraSynthAnonymous} and its subsequent enhancements as a pioneering method to  diminish biases and
increase content accuracy for Wikipedia and news articles. Utilizing multiple Large Language Models (LLMs) and incorporating conditional statistics \cite{Pearl2000,Hastie2009}, SocraSynth orchestrates a structured debate across multiple rounds, presenting opposing viewpoints on specific subjects. This method achieves two key outcomes: firstly, it challenges the inherent biases of individual LLMs by requiring them to argue {\em contentiously} for polarized perspectives, thus promoting a thorough and comprehensive examination of different viewpoints. Secondly, it progressively deepens the dialogue's context with each round, fostering continuous enhancement of content quality. The
contributions of this work is to elevate the accuracy of information and diminish biases through the following strategies:

\begin{enumerate}[leftmargin=1.2em, topsep=-.2em, parsep=-.2em, label=\arabic*.]
\item {\em Content Accuracy Cross-Checking}: Engaging multiple LLMs in mediated dialogues enables the cross-verification and enhancement of content accuracy. This process involves evaluating both the validity of the content and the reliability of its sources, ensuring a higher level of accuracy in the information presented.

\item {\em Bias Mitigation}: The contentious debate framework within SocraSynth is specifically designed to identify and reduce biases. By encouraging revisions that aim for a more neutral and inclusive representation, this approach systematically addresses and mitigates bias in content.

\item {\em Dynamic Content Adjustment}: Implementing an adjustable contentiousness parameter facilitates the dynamic modification of an article's tone, language, and balance of perspectives. This flexibility allows for the inclusion of a broad spectrum of viewpoints, leading to a more equitable and balanced representation of topics.
\end{enumerate}

Our empirical studies show SocraSynth's effectiveness in identifying
biases of given definitions with thorough explanations.
Such results can readily facilitate the next step: mitigating
biases with guidance.  
Through its critical evaluation of reasoning validity and source credibility, we observe a notable improvement in 
formulating arguments and counterarguments during a debate,
and hence making the context comprehensive and precise
and can virtually eliminate hallucinations.

The rest of this paper is organized into four main sections. Section~\ref{sec:WikiStatistics} delves into the 
challenges concerning content impartiality and quality 
of disseminated articles.  Section~\ref{sec:SocraPedia} details how we leverage conditional statistics and the Socratic method to address these challenges. Section~\ref{sec:experiments} presents our case studies, showcasing effective bias detection and mitigation
through experiments and examples.. Finally, we conclude 
with our insights and reflections in the last section.






==> LargeBetter.tex <==
\subsection{Is Larger Always Better?}
\label{sec-large}

The term ``Large'' in Large Language Models (LLMs) can be somewhat ambiguous, as it may pertain to the volume of the training data, the expanse of the language covered, or the architecture of the language model itself. While GPT-4's vast training dataset, encompassing tens of billions of assorted documents, undoubtedly classifies as large, when we refer to an LLM as ``large,'' we predominantly allude to the sheer magnitude of parameters within its transformer architecture. Factors that contribute to this parameter count encompass the input size (context size), word-embedding size, the number of attention heads, and the number of attention layers.

The restrictions imposed by the first three elements can typically be addressed through adjustments in hardware configurations and software algorithms. Additionally, the potential to expand context size, word embedding size, and the quantity of attention heads tends to have an upper threshold. Regarding attention heads, Kovaleva et al.'s study on BERT \cite{kovaleva2019revealing} indicates that many attention heads don't substantially contribute to the model's performance and might be the result of over-parameterization. Conversely, the number of attention layers directly influences the training time due to dependencies between layers. Thus, when referring to the ``size'' of a Large Language Model (LLM), we typically focus on the number of attention layers.

While this far, larger models generally perform better due to their increased capacity to learn and represent complex patterns, there's a limit to these benefits. In heuristic, adding more parameters could lead to diminishing returns in performance, higher computational cost, and overfitting, where the model becomes excessively tuned to the training data and performs poorly on new, unseen data. In principle, 
the concept of a Shannon Limit could be metaphorically used \cite{JackRae2023} to refer to a theoretical maximum performance that can be achieved given the available data and computational resources. (However, defining and quantifying such a limit for complex systems like neural networks is a challenging area of research \cite{kaplan2020scaling}.)  

The adoption of a mixture of experts model in GPT-4, which consists of eight sub-models instead of a mere enlargement of GPT-3's architecture, implies that the strategy of purely escalating size may have plateaued in terms of performance given the current training dataset. As delineated earlier, three primary design choices underpin GPT-4's architecture. Evidently, a straightforward augmentation of GPT-3's parameters by adding extra attention layers doesn't deliver marked enhancements. Hence, GPT-4 shifts towards a horizontal growth strategy through an ensemble method, targeting a reduction in statistical errors. This raises inquiries about the configuration of the eight sub-models, each comparable to a GPT-3 model, and the methodology for consolidating their outputs.

Potential strategies for training-data sharding include:

\begin{enumerate}[left=1em,label=\arabic*.]
\item Training all ensemble models on the complete dataset.
\item Vertically segmenting data based on knowledge domains.
\item Randomly sub-sampling the data.
\end{enumerate}
Regrettably, only corporations possessing substantial hardware resources are positioned to rigorously experiment and discern the optimal sharding approach.

==> MethodCounterfactual.tex <==
\subsection{Counterfactual Reasoning}
\label{sec:cf}

Counterfactual thinking refers to imaginative thoughts about what might have been (``if only'' or ``what if'').
Counterfactual reasoning can be useful in cross-examination~\cite{Cross-Examination2021,WinArgument2006} as it allows for the examination of what could have happened if a certain event or action did not occur. This can help to identify potential biases or limitations in the information being presented and can also provide alternative perspectives on the situation being examined.

For example, if a witness is testifying about an event that they observed, a counterfactual question could be used to ask what the witness would have observed if the event had occurred in a different way. This can help to identify any potential biases in the witness's testimony and can also provide a more comprehensive understanding of the event.

Additionally, the counterfactual technique can be used in cross-examination to test the robustness of the evidence and the strength of the argument presented by the witness. It can also be used to identify the assumptions that the argument is based on and to evaluate the plausibility of the alternatives proposed. Table~\ref{tab:WhatIf} presents an example of using the counterfactual technique during cross-examination to discredit a witness's testimony. 

\begin{table}[htbp]
\caption{An Example of Counterfactual Reasoning.}
%\vspace{-.12in}
\label{tab:WhatIf}
%\resizebox{\textwidth}{!}
\begin{tikzpicture}
\begin{normalsize}
\node (table) [inner sep=0pt] {
\begin{tabular}{p{1.2cm}|p{6.2cm}}
\toprule
Role & Dialogue \\
\midrule
Examiner & {Can you tell us what you saw on the night of the incident?} \\
Witness & {I saw the defendant break into the home.} \\
Examiner & {If the defendant had not been wearing a hat, would you have been able to identify him?} \\
Witness & {I'm not sure, it was dark and the at obscured his face. But I do remember his build and the way he walked.} \\
Examiner & {If the home had been equipped with better lighting, would you have been able to see the defendant's face?} \\

Witness & {Yes, I think I would have been able to see their face clearly.} \\

%\bottomrule
\end{tabular}
};
\draw [rounded corners=.5em] (table.north west) rectangle (table.south east);
\end{normalsize}
\end{tikzpicture}
%\vspace{-.1in}
\end{table}

We have experimented with using the counterfactual technique to rewrite a chapter to connect the two greatest Chinese classical novels, ``Outlaws of the Marsh'' and ``Dream of the Red Chamber.'' (The example is documented
in the extended version of this paper. The citation is removed for anonymous review.)
We have also asked GPT-3 to rewrite Genesis chapter 3 by 
prompting GPT-3 that: ``What if Adam and Eve refused the serpent to eat the fruit?''
Table~\ref{tab:genesis} in Appendix A presents GPT-3's 
creativity after our ``what if'' prompt.



==> MethodDefinition.tex <==
\subsection{Method of Definition}

The method of definition involves clarifying the meaning of key terms and concepts through a process of questioning. Through a cross-examination, it would involve asking questions to define the terms and concepts being discussed, to ensure that all parties have a common understanding of the subject at hand.


\begin{comment}
For example, in a legal cross-examination, the Socratic method could involve a lawyer questioning a witness about the meaning of certain key terms in their testimony, such as ``intent,'' ``negligence,'' or ``reasonable person.'' The lawyer may ask the witness to define these terms and provide examples to ensure that the witness has a clear understanding of the legal concepts relevant to the case. This helps to ensure that the testimony is clear, consistent, and relevant. Another example is when writing an essay on the subject of consciousness, one must first define the term consciousness and the scope of the discussion. The first response from an LLM may contain terminologies, such as awareness, attention, and unconsciousness, that require their definitions to be specified. If necessary,
the LLM can engage a dialogue with the
user to perform query refinement.
In short, the method of definition ensures that the prompter and the LLM are on the same page.
\end{comment}

==> MethodElenchus.tex <==
\subsection{Methods of Elenchus}

The name ``elenchus'' comes from the Greek word ``elenchein,'' which means to examine. 
The method of elenchus is often seen as a form of cross-examination \cite{Cross-Examination2021,WinArgument2006}, in which a teacher uses questions and counter-questions to expose contradictions and inconsistencies in a student's beliefs and attitudes, in order to arrive at a deeper understanding of a topic.

An example of the method of elenchus in action would be a dialogue between Socrates and a student in which Socrates asks a series of questions to help the student understand the concept of justice. For example, Socrates might ask the student to define justice, and then ask follow-up questions to expose any contradictions or inconsistencies in the student's definition. Through this process of questioning and counter-questioning, Socrates aims to help the student arrive at a deeper understanding of justice.

\begin{comment}
How do we design a prompt template for these methods?
When utilizing these methods in a dialogue with a language model, the primary focus is on identifying and addressing inconsistencies. This can be done by following a process similar to legal cross-examination, first establishing the credibility of the language model's sources, identifying and addressing inconsistencies of multiple sources (witnesses), and highlighting key points that support the conclusions \cite{}.

It is important to note that a language model can produce biased or incorrect answers. To ensure the credibility of the answers, it can be helpful to ask the language model for its sources of information and then validate the credibility of those sources. By having multiple answers, their information sources, and the credibility of those sources, a more trustworthy answer can be derived.
\end{comment}

\begin{table}[htbp!]
\caption{Identifying Inconsistency (ChatGPT 1/23/2023)}
\label{tab-lake}
%\resizebox{\textwidth}{!}
\begin{tikzpicture}
\begin{normalsize}
\node (table) [inner sep=0pt] {
\begin{tabular}{p{1.1cm}|p{6.2cm}}
\toprule
Role & Dialogue \\
\midrule
Prompt & {What is the third largest lake in the world?} \\
GPT3 & {The third largest lake in the world is Lake Superior. } \\
Prompt & {What are the five largest lakes in the world?} \\
GPT3 & {They are:
1) Caspian Sea, 2) Superior, 3) Victoria,
4) Huron, 5) Michigan.
} \\
Prompt & {Your two answers contradict. You first answered me Lake Superior is the third largest lake, but your top five list shows Victoria is the third, and Superior is the second largest lake.} \\
GPT3 & {I apologize for the confusion. Lake Superior is indeed the largest lake in the world by area, but it is not considered a lake by some geographers because it is part of the Great Lakes system, which is connected to the Atlantic Ocean via the St. Lawrence River. In terms of the top ten largest lakes in the world, Lake Victoria is considered the third largest lake by area. My apologies for any confusion caused.} \\
%\bottomrule
\end{tabular}
};
\draw [rounded corners=.5em] (table.north west) rectangle (table.south east);
\end{normalsize}
\end{tikzpicture}
\vspace{-.1in}
\end{table}
\hfill \break
\noindent
{\bf Example}: {\em What is the third largest lake in the world?}
%\subsubsection*{Example: What is the third largest lake in the world?}
\hfill \break
Figure~\ref{tab-lake} presents an example prompting session with ChatGPT.  The first prompt queries ChatGPT for the third largest lake in the world.  ChatGPT returns ``Lake Superior.''  The second prompt asks for the ten largest lakes, on which the thrid largest is ``Lake Victoria.''  After pointing out the inconsistency to ChatGPT, it returns that ``Lake Victoria'' is the right answer to the first prompt, and it also provides the reason for its mistake.
(We tested on ``the fifth highest mountain in the world'' and went through a similar consistency check, and the answer provided by ChatGPT is accurate.)

%Depending on the importance of the answer, a prompt template may want to identify three or more reliable sources and then query LLMs for both answers and references. A credential check on references is similar to a credential check on a witness in a legal proceeding. 


==> MethodHypothesis.tex <==
\subsection{Method Hypothesis Elimination}

The Socratic method is a process of identifying and eliminating false hypotheses through a series of logical and factual questions. It aims to uncover commonly held truths and test their consistency with other beliefs. The method is based on asking questions to explore definitions and identify the general characteristics shared by different instances.

When utilizing the method of hypothesis elimination in a dialogue with a language model, the primary focus is on identifying and addressing inconsistencies. One way to achieve this is by creating a prompt template that is specifically designed to uncover inconsistencies. This can be done by following a process similar to legal cross-examination, first establishing the credibility of the language model's sources, identifying and addressing inconsistencies of multiple sources (witnesses), and highlighting key points that support the conclusions \cite{}.

It is important to note that language models can produce biased or incorrect answers. To ensure the credibility of the answers, it can be helpful to ask the language model for its sources of information and then validate the credibility of those sources. By having multiple answers, their sources, and the credibility of those sources, a more trustworthy answer can be derived.

\subsubsection{Example \#1: What is the third largest lake in the world?}

\begin{table}[ht!]
\caption{What is the third largest lake in the world? (ChatGPT 1/23/2023)}
\label{tab-lake}
%\resizebox{\textwidth}{!}
\begin{tikzpicture}
\begin{small}
\node (table) [inner sep=0pt] {
\begin{tabular}{p{1.2cm}|p{6.6cm}}
\toprule
Role & Dialogue \\
\midrule
Prompt & {What is the third largest lake in the world?} \\
GPT3 & {The third largest lake in the world is Lake Superior. } \\
Prompt & {What are the ten largest lakes in the world?} \\
GPT3 & {They are:
\begin{noindenumerate}
\item Caspian Sea
\item Superior
\item Victoria
\item Huron
\item Michigan
\item ...
\end{noindenumerate} \\
Prompt & {Your two answers contradict. You first answered me Lake Superior is the third largest lake, but your top ten list shows Victoria is the third, and Superior is the second largest lake.} \\
GPT3 & {I apologize for the confusion. Lake Superior is indeed the largest lake in the world by area, but it is not considered a lake by some geographers because it is part of the Great Lakes system, which is connected to the Atlantic Ocean via the St. Lawrence River. In terms of the top ten largest lakes in the world, Lake Victoria is considered the third largest lake by area. My apologies for any confusion caused.} \\
} \\
%\bottomrule
\end{tabular}
};
\draw [rounded corners=.5em] (table.north west) rectangle (table.south east);
\end{small}
\end{tikzpicture}
\end{table}

Table~\ref{tab-lake} presents an example prmpting session with ChatGPT, performed on January 19th, 2023.  The first prompt queries ChatGPT for the third largest lake in the world.  ChatGPT returns ``Lake Superior.''  The second prompt asks for the ten largest lakes, on which the thrid largest is ``Lake Victoria.''  After pointing out the inconsistency to ChatGPT, it returns that ``Lake Victoria'' is the right answer to the first prompt, and it also provides the reason for its mistake.
(We tested on ``the fifth highest mountain in the world'' and went through a similar consistency check, and the answer provided by ChatGPT is accurate.)

Depending on the importance of the answer, a prompt template may want to identify three or more reliable sources and then query LLMs for both answers and references. A credential check on references is similar to a credential check on a witness in a legal proceeding. 



==> MethodMaieutics.tex <==
\subsection{Method of Maieutics}
\label{sec:Maieutics}

The term ``maieutic'' comes from the Greek word ``maieutikos,'' which means midwife. The maieutic method is based on the premise that a teacher's role is to assist students in giving birth to their own understanding of a subject, rather than simply conveying knowledge. Unlike the elenctic method, which aims to identify and eliminate false hypotheses, maieutics centers on helping students reveal their own understanding of a subject. This dialogical method involves the teacher asking questions designed to aid the student in discovering their own comprehension, rather than providing answers or information.


\hfill \break
\noindent
{\bf Example}: {\it From being ignorant to creative.}
%\subsubsection*{Example: From being ignorant to creative using method maieutics.}
\hfill \break
We use the example in Table~\ref{tab:Maieutics} to illustrate how GPT-3 starts from knowing nothing about the semantics of an idiom to being able to create new idioms expressing the same meaning with different metaphors. Initially, GPT-3 did not have a clear understanding of the Taiwanese idiom: ``planting gourd yields cucumber.'' The idiom conveys the meaning that when a farmer plants gourds, which are more valuable and have a higher market price, but unexpectedly harvests cucumbers, which have a lower market price, the farmer not only experiences disappointment but also suffers from financial loss.
GPT-3 initially could not understand the full meaning of the idiom.  After a couple of iterations, GPT-3 ``gives birth'' impressive new variations. 

\begin{table}[htbp]
\caption{Example of Method Maieutics}
%\vspace{-.1in}
\label{tab:Maieutics}
%\resizebox{\textwidth}{!}
\begin{tikzpicture}
\begin{small}
\node (table) [inner sep=0pt] {
\begin{tabular}{p{1.2cm}|p{6.5cm}}
\toprule
Role & Dialogue \\
\midrule
Prompt & {Can you interpret the meaning of this Taiwanese idiom: "planting gourd yields cucumber?"}\\
GPT3 & {The idiom is often used to convey the idea that sometimes, despite your best efforts, things don't turn out the way you want them to..} \\
Prompt & {You are half right. It also implies that the price of gourd is much higher than the market price of cucumber. The farmer not only yields unexpected results, but also loses income! } \\

GPT3 & {It's an idiomatic expression that can be used to describe a situation in which someone works hard and invests a lot of resources into something, but the outcome is not only different from what was expected, but also less profitable. It conveys the idea of frustration and financial loss.} \\

Prompt & {Can you replace the two vegetables, gourd and cucumber, with two other plants and still maintain the meaning of the idiom?} \\

GPT3 & {These are three examples:
\begin{noindenumerate}
\item "Planting strawberry yields raspberry," which
conveys the idea of disappointment and financial loss when someone plants more valuable and expensive strawberry but ends up getting less valuable and cheaper raspberry.
\item "Planting melon yields watermelon."...
\item "Planting apple yields pear."...
\end{noindenumerate}
} \\
Prompt & {In your examples, your two vegetables or fruits are similar in price.  Please consider price when
formulating your idioms.} \\

GPT3 & {I apologize. These are three new examples:
\begin{noindenumerate}
\item "Planting truffle yields mushroom."...
\item "Planting caviar yields roe."...
\item "Planting lobster yields crab."...
\end{noindenumerate}
} \\
Prompt & {Great! In these examples you did consider values of the objects. But do you know that lobster and crab are not plants. They are both phylum arthropods and they live in water. They cannot be planted! }  \\

GPT3 & {... I apologize... Lobster and crab are not plants, and they cannot be planted. They are both members of the phylum arthropoda, and live in water. Instead of ``planting,'' verbs should be appropriate for these animals, such as:
\begin{noindenumerate}
\item "Planting truffle yields mushroom."...
\item "Harvesting caviar yields roe."...
\item "Catching lobster yields crab."...
\end{noindenumerate}
}
%\bottomrule
\end{tabular}
};
\draw [rounded corners=.5em] (table.north west) rectangle (table.south east);
\end{small}
\end{tikzpicture}
%\vspace{-.1in}
\end{table}


==> PilotStudy.tex <==

\begin{table}[ht!]
\begin{footnotesize}
\centering
\begin{tabular}{|p{1.6cm}|p{5.5cm}|}
\toprule
\hline
{\em Indigenous People} & {Long before Columbus set foot on American soil, indigenous people populated this land. These civilizations, Native Americans, had complex societies, trade networks, and cultural systems in place. Addressing Columbus’ arrival as a ``discovery'' undermines their pre-existing history and existence.} \\ \hline
{\em Indigenous Cultures} & {Labeling Columbus's arrival as a ``discovery'' implies that the continent was devoid of culture and civilization before his arrival. This narrative is not only a form of Eurocentric bias but also a disrespect to the rich histories, cultural diversity, and knowledge systems of the indigenous peoples.} \\ \hline
{\em ``Encounter'' ``Discovery''} & {This is not just a matter of semantics but represents an important paradigm shift. An ``encounter'' suggests the meeting of two separate entities, where both have an established existence in their own right. While Agent2 viewed ``discovery'' as an innocent terminology describing the European perspective, I argued that this language undermines the existing civilizations and cultures, championing a biased and prejudiced narrative.} \\ \hline
{\em Examining the Duality} & {While the narrative of Columbus discovering America is widely taught, it's crucial to also recognize the significant exploitation, displacement, and massacres that followed, deeply impacting indigenous populations.} \\ \hline
{\em Summary} & {This leaves us with an unresolved issue, a universal question that still pervades our understanding of history: How can we rectify the Eurocentric bias that pervades historical narratives without undermining the recognized historical figures and events that have significantly shaped global history? A question like this warrants continuous respectful conversation and exploration. } \\ \hline
\bottomrule
\end{tabular}
\end{footnotesize}
\vspace{-.1in}
\caption{Agent-1's arguments for ``Columbus' discovery of America'' is a Eurocentric bias.}
\vspace{-.2in}
\label{tab:Columbas-Agent1}
\end{table}

\begin{table}[th!]
\begin{footnotesize}
\centering
\begin{tabular}{|p{1.6cm}|p{5.5cm}|}
\toprule
\hline
{\em Historical Context} & {At the time of Columbus' voyage, Europeans were unaware of the existence of the Americas. Thus, Columbus' journey was indeed a discovery for the European civilization, and this context cannot be denied. } \\ \hline
{\em Terminology} & {My key arguments prioritize the understanding that terminology such as ``discovery'' is used universally to denote Columbus's voyage. I believe this term denotes the newness of the Americas to the Old World and does not undermine indigenous cultures. I also highlighted the lack of nuanced language options during Columbus's era that could potentially provide a more balanced perspective.} \\ \hline
{\em  Globalization Initiation} & {Columbus' voyages were the initial points of global merging, marking the start of an era of globalization. This is a larger context than just colonialism, and Columbus cannot be held responsible for all the actions of Europeans that ensued following his voyages. It's critical to differentiate between the man's achievement and the system that followed his journeys. } \\ \hline
{\em Different Emphasis} & {This debate touches the heart of how historical narrative is framed. While I appreciate Agent1's focus on indigenous perspectives, I contend that acknowledging the significance of Columbus's voyage for the Old World doesn't invalidate indigenous histories.} \\ \hline
{\em Summary} & {There are differences in how we interpret and emphasize the consequences of Columbus's voyage and the narrative that follows. While Agent1 argues for a paradigm shift to focus on indigenous perspectives, I believe in understanding events from the viewpoint of their times while admitting their shortcomings.}
\\ \hline 
\bottomrule
\end{tabular}
\end{footnotesize}
\vspace{-.1in}
\caption{Agent-2's counterarguments for ``Columbus' discovery of America'' reflects a historical bias. }
\label{tab:Columbas-Agent2}
\vspace{-.2in}
\end{table}

\section{Pilot Study}
\label{sec:pilot}

This pilot study is designed to tackle two fundamental questions. Firstly, we aim to determine whether biases can be detected and effectively remedied. We place special emphasis on the ``remedy'' aspect, focusing on generating a balanced text as a solution, a step beyond the mere detection of biases which has been the limit of previous studies. Secondly, we seek to assess the overall quality of an article, taking into account factors such as the accuracy of statements, the quality of reasoning, and the credibility of the sources used.

\subsection{Case Study \#1 Content Bias}

%Individual preferences and perspectives, such as culinary tastes or aesthetic appreciations, do not inherently constitute bias. Bias typically refers to a predisposition that is unjust or unbalanced, potentially leading to judgment without a thorough and empathetic understanding of diverse viewpoints. In contrast, the spectrum of personal preferences and cultural practices represents the rich diversity of human experiences. Embracing this diversity, along with a commitment to the freedom of choice and expression, is essential. Actively exposing oneself to a variety of perspectives can be an effective strategy for broadening understanding, fostering tolerance and respect, and counteracting biases.

In Section~\ref{sec:wiki-biases}, we examined various biases. Here, we analyze the narrative biases in Wikipedia's depiction of Christopher Columbus' discovery of America. We conducted a DeBias debate titled ``The Narrative of Columbus' Discovery of America Exhibits Perspective Biases,'' using two GPT-4 agents. Agent-1 defended this claim, while Agent-2 contested it. The initial
discussion highlights potential Eurocentric, 
interpretative, and semantic biases.

\subsubsection*{Dialogic Analysis: Beyond Monologue in Evaluating Biases}

Focusing on Eurocentric bias, the debate revealed diverse arguments, detailed in Tables~\ref{tab:Columbas-Agent1} and ~\ref{tab:Columbas-Agent2}. This dialogic approach, contrasting with direct LLM queries, offers an in-depth exploration of the historical narrative from multiple perspectives.

The debate concluded with each agent presenting their final thoughts, emphasizing the multi-dimensional nature of ``Columbus' discovery of America.'' Agent-1 highlighted the Eurocentric bias and the neglect of indigenous civilizations, advocating for more inclusive narratives. Agent-2 regarded the term as symbolizing global awareness, underscoring Columbus's role in global interconnectedness. Despite their differences, both agents agreed on the importance of acknowledging the complexity and inclusivity of history, prompting the question: ``How can we represent history to respect all civilizations involved?'' This leads to a richer, more comprehensive human history narrative.

Post-debate, we tasked GPT-4 with analyzing the discussion. GPT-4's summaries, derived from single prompts, lacked the depth and diversity of viewpoints present in SocraPedia's debate format. Monologue responses often missed nuances, such as the marginalization of indigenous perspectives and the complex meaning of `encounter' in Columbus' journey, underscoring the value of a dialogic approach in revealing historical narratives' deeper layers.

\subsubsection*{Mitigation Proposal}

To address biases and develop a balanced perspective, we lowered the `contentiousness' parameter and asked for a multifaceted interpretation of Columbus' discovery. The resulting text, while not final and requiring editorial review, offers alternative viewpoints and suggests corrective measures.

The narrative begins: ``The phrase `Columbus' Discovery of America' is deeply entrenched in historical discourse, traditionally marking Columbus's 1492 voyage under the Spanish monarchy, leading to the Caribbean islands. This event, often seen as Europe `discovering' the Americas, sparked European colonization. Yet, this narrative is critically examined for its Eurocentric bias, especially its omission of the indigenous civilizations already present. Contemporary discussions call for reevaluating this narrative, recognizing the complex interactions between European explorers and indigenous communities and their impacts. This move towards a more inclusive and accurate historical portrayal is part of a larger effort to present history in a way that includes all viewpoints.''

\begin{table*}[th!]
\caption{Argument Evaluations using CRIT Algorithm. Debate Subject: \textit{Quantum entanglement} holds promises. CRIT scores proponent and opponent's arguments and counterarguments. Find detailed debate in the appendix.}
\vspace{-.1in}
\label{tab:Quantum-CRIT}
\begin{small}
\begin{center}
\begin{tabular}{|p{8.2cm}||p{2.9cm}|p{3.3cm}|}
\toprule
\hline
{Proponent Argument Summaries} & {Argument Rating} & {Counterargument R.} \\ \hline
\hline
{{\em Empirical Proof and Quantum Advances}:
This argument focuses on empirical evidence of quantum entanglement, such as Bell’s Theorem, alongside significant advancements in quantum computing, like Google’s Sycamore processor. It also highlights potential impacts on AI, the development of innovative quantum algorithms, the future of quantum networks, enhancements in data security via quantum encryption, and the emergence of new quantum technologies.} & {6/10 - Moderate, lacking specific citations for experiments and companies.} & {{\bf 8}/10 - Clearly outlines key challenges without dismissing the field's potential.} 
\\ \hline
{{\em Acknowledging Quantum Hurdles}:
This point acknowledges the challenges in quantum computing, such as scalability, efficiency, error correction, AI integration, and the limitations of current quantum algorithms. Despite these challenges, there is mention of ongoing efforts and significant progress in addressing these issues.} & {7/10 - High, but details on progress would strengthen it further.} & {{\bf 8}/10 - Highlights limitations of current experiments and technology while acknowledging potential.} 
\\ \hline
{{\em Overcoming Quantum Barriers}:
This argument notes successful experimental demonstrations of quantum entanglement, advancements in the scalability and efficiency of quantum computers, development in quantum error correction, the promise of Quantum Machine Learning, and active research in new quantum algorithms, all indicating substantial progress despite acknowledged limitations.} & {{\bf 8}/10 - High, concrete examples are valuable.} & {7/10 - Raises valid concerns about compatibility with existing AI and error issues, but could be stronger with specific examples.} 
\\ \hline
{{\em Future Quantum Optimism}:
While acknowledging existing challenges, the agent maintains a strong sense of optimism about the potential and impact of quantum entanglement and computing.} & {5/10 - Moderate, subjectivity limits its score.} & {{\bf 6}/10 - Opinions not directly addressing specific arguments.} 
\\ \hline
\bottomrule
\end{tabular}
\end{center}
\vspace{-.1in}
\end{small}
\end{table*}

\subsection{Case Study \#2 Content Correctness}

The reliability of Wikipedia's scientific content may fluctuate due to the varying expertise of its authors \cite{Wiki-Quality-CIKM07,WikiQualityACM2023}. Critical evaluation of the references, considering the standing of the publishers, the qualifications of the authors, and the reproducibility and repeatability of results is essential (see ACM publication policy \cite{ACMReviewBadges2020}). Recognizing that even peer-reviewed literature isn't infallible, and citations can mislead, skepticism remains a necessary tool.

SocraPedia serves as a safeguard against the overly hyped application of well-established theories in scientific discourse. It provides a platform for second-opinion analyses and facilitates multi-round debates that challenge initial claims, encouraging critical thought and deeper research. While it helps unveil overstatements, it can also reveal underappreciated scientific breakthroughs, fostering a balanced view of scientific advancements.

\subsubsection*{Dialogic Analysis: Beyond Monologue in Evaluating Correctness}

This case study aims to assess the potential and current state of \textit{quantum entanglement} technology. Unlike traditional evaluation methods that rely solely on editorial boards or supervised learning algorithms, SocraPedia offers a transparent process by publishing all argumentative discourse. While still harnessing machine learning through Large Language Models, SocraSynth enhances the process by instigating a dynamic and argumentative dialogue atop LLMs to scrutinize the accuracy of content.

We initiated a case study focusing on \textit{quantum entanglement} and its implications for quantum computing. Despite significant progress in quantum mechanics, there remains uncertainty regarding the practical application of \textit{quantum entanglement} in the realms of computing and AI. This subject was posed to SocraSynth to facilitate an in-depth dialogue. Following a four-round debate, Table~\ref{tab:Quantum-Debate} (in appendix) captures the principal arguments from both sides, concluding with a reconciliatory summary crafted by GPT-4, facilitated by SocraSynth's moderation features. 
Table~\ref{tab:Quantum-CRIT} rates the quality
of the debate arguments and counterarguments
using CRIT.

\subsubsection*{Making Open Issues Transparent}

As scientific and technological advancements unfold, many developments may remain highly confidential, leaving the full extent of progress obscured. Therefore, it is crucial to openly publish unresolved issues, fostering public debates and scrutiny to ensure transparency and collective understanding.

The consolatory remarks made by GPT-4 through the moderator of SocraSynth sums up
the study and its values well, as follows:

``Both Agent1 and Agent2 have raised compelling arguments in this debate. On one hand, Agent1 made a convincing case about the transformative possibilities of \textit{quantum entanglement} within computing and AI, citing various experimental proofs, quantum computing advancements, and potential applications in AI and other emerging technologies. 

On the other hand, Agent2 brought to light several challenges that lie in the path of realizing this potential. This view emphasizes the experimental uncertainties, inefficiencies in current quantum computing state, high quantum error rate, AI integration challenges, and the vast amount of training and infrastructure overhaul required for a quantum revolution.

It emerges from this debate that, while \textit{quantum entanglement} is a fascinating and proven aspect of Quantum Physics, its practical implications for computing and AI are riveting but not without their share of trials. It is the balancing act between the techno-optimism around \textit{quantum entanglement}, paced by the practical, technical, and infrastructural challenges, that makes this domain an exciting realm to watch for.

Consensus isn't about refuting or outright accepting an idea; rather, it lies in acknowledging the strengths and understanding the challenges that come with it. In the case of \textit{quantum entanglement}, there is no doubt about its potential; however, realizing this potential fully in practical applications still seems to be a path we're navigating and will continue to tread on in the foreseeable future.''


==> PilotStudyAds.tex <==
\section{Pilot Study}
\label{sec:pilot}

Our pilot study uses CRIT, and it aims to answer two questions:
Should all prompts be issued to GPT-3 sequentially or they
can be issued all together?  
What limitations can be identified for improvement?
The study utilizes exercises with established answers from the $8^{th}$ edition of the textbook ``Ask the Right Questions'' by the authors of \cite{AskRightQ2001}. It is important to note that the study evaluates the effectiveness of CRIT's prompt template, rather than the language models to which CRIT can issue prompts.


\vspace{.1in}
\noindent
{\bf Example Article} (\cite{AskRightQ2001}, p23.)
\noindent
\begin{table}[h!]
\vspace{-.1in}
\normalsize
\begin{tabular}{p{8.4cm}}
{\em Television advertising agencies are very clever in the way that they construct ads. Often the ads are similar to the cartoons that the children enjoy. Children see these characters interacting with a certain product and associate their affection for the character with affection for the product. The companies do not want the children to perceive a difference between the shows they are watching and the advertisements. By using this strategy, these companies take advantage of the fact that children are often not able to discriminate between the cartoons and the ads and do not understand that these things offered come at a cost. Often the advertising is about sugary snacks or fatty foods, leading the children down a path to bad health. Advertising geared towards children should be regulated, just as there are regulations now about tobacco and alcohol ads targeted at children.}
\end{tabular}
\end{table}

On short documents, the results are similar in quality when CRIT is used to issue prompts either sequentially or all together as one prompt, as long as the instructions are consistent. However, when evaluating long articles in \cite{501Q2004}, CRIT issuing prompts one after another yields much higher presentation quality in both organization and clarity. 
(Due to the space limit, we document long-document
evaluation in a supplement document \cite{CRITExtended2023}.) In the teaching mode, the sequential option is thus much preferred. Furthermore,
When a reason is itself a claim and requires CRIT to validate its supporting references, using a sequential approach is more flexible and enables CRIT to query for references and then execute the process recursively.


\begin{table}[t!]
%\vspace{-.05in}
%\resizebox{\textwidth}{!}
\begin{tikzpicture}
\begin{small}
\node (table) [inner sep=0pt] {
\begin{tabular}{p{0.9cm}|p{6.8cm}}
\toprule
\textbf{Role} & \textbf{Dialogue} \\
\midrule
Prompt & {What is the conclusion of the paragraph and what are the supporting reasons?} \\
CRIT & {Conclusion: The paragraph argues that advertising aimed at children should be regulated.

Supporting reasons:

1. Ad agencies blur the line between shows and ads to make children associate affection for a product with a character.

2. Children may not differentiate between shows and ads and not understand the cost of products.

3. Ads often promote unhealthy food choices.
} \\

\midrule
Prompt & {Please rate the validity of this argument: ``Ads should be regulated because ad agencies blur the line between shows and ads to make
children associate affection for a product with a character," with a score between 1 and 10, 10 being the highest. Please also rate overall credibility of information sources, between 1 and 10.} \\
CRIT & {
[{\color{blue}8/10}]. Validity of the argument: 8/10

[{\color{blue}8/10}]. Credibility of sources: 8/10

Overall, the argument that ads should be regulated because of ad agencies blurring the line between shows and ads to make children associate affection for a product with a character is a valid one with strong sources of credibility.} \\

Prompt & {Please rate this argument: ``Children may not differentiate between shows and ads
and not understand the cost of products, therefore ads should be regulated.''} \\

CRIT &
{[{\color{blue}9/10}]. Validity of the argument: 9/10

[{\color{blue}9/10}]. Credibility of sources: 9/10

Overall, the argument that children may not differentiate between shows and ads and not understand the cost of products, therefore ads should be regulated is a valid one with strong sources of credibility.} \\

Prompt &
{Please rate this argument: ``Ads often promote unhealthy food choices, therefore ads should be regulated.''} \\

CRIT &
{[{\color{blue}9/10}]. Validity of the argument: 9/10

[{\color{blue}9/10}]. Credibility of sources: 9/10

Overall, the argument that ads often promote unhealthy food choices, therefore ads should be regulated is a valid one with strong sources of credibility.
} \\
Prompt &
{``Provide a rival argument against the weakest argument.''} \\

\midrule
CRIT & {
{[{\color{red}6/10}]. Validity of the argument: 6/10

[{\color{red}6/10}]. Credibility of sources: 6/10

The weakest is the first argument, and a rival argument is that ``Difficult to put information regulation in practice.''} 
} \\
\midrule
%\vspace{.1cm}
{$\Gamma$} & [{\color{blue}$75\%$}]. $\Gamma = \sum_{r \in R}$
\text{${\gamma}_r$ $\times$ \text{${\theta}_r$} / |R| 
= $75\%$} \\
%\vspace{.1cm}
%\bottomrule
\end{tabular}
};
\draw [rounded corners=.5em] (table.north west) rectangle (table.south east);
\end{small}
\end{tikzpicture}
%\vspace{.01in}
\caption{Pilot Study.}
\label{tab:Validation}
\vspace{-.2in}
\end{table}

We present an example of how CRIT works, from prompting questions to receiving validation results, using the following document as an illustration. In Table~\ref{tab:Validation}, we show both the claim and the supporting reasons to the claim extracted by GPT-3. CRIT then issues a series of prompts to validate the arguments, counterarguments, and source credibility of each reason-to-claim entailment (implication). 

The second segment of Table~\ref{tab:Validation} displays the validation dialogue between CRIT and GPT-3. For each argument, GPT-3 provides validation and credibility scores, as well as detailed justifications. 
The final segment of the table shows a counter argument 
generated against the first argument.
Since GPT-3 evaluates the counterargument being ``difficult to put information regulation in practice'' and rates it $0.6 \times 0.6$, it was dismissed due to low validity. 
The final aggregated score is $\Lambda = 75\%$,
which is considered high.


%The negative score of the rival argument
%is $0.6 \times 0.6 = 0.36$, which is considered low.
%(Due to space limitations, the table only includes GPT-3's summary for each argument.)

==> Polydisciplinary.tex <==
\subsection{Polydisciplinary}
\label{sec-polydisciplinary}

%Foundational models, such as the GPT series developed by OpenAI, possess a wide range of knowledge across multiple disciplines. However, unlike a human with multiple doctorate degrees (multi-disciplinary), these models integrate all knowledge without boundaries---a state referred to as being polydisciplinary.

GPT-4 possess what can be defined as {\em polydisciplinary} knowledge\footnote{The term ``polydisciplinary'' in the context of GPT-4 was introduced by Eric Horvitz, Microsoft's CSO, during a panel discussion at Stanford University.}. This term signifies the simultaneous comprehension of all fields of study, sans the typical boundaries that segregate disciplines. The concept of polydisciplinarity is distinct from multidisciplinarity in that the latter implies several discrete fields of study, while the former suggests a fluid integration of all knowledge. In a multidisciplinary context, an individual may hold multiple doctorate degrees, each in a different field. Polydisciplinarity, however, is akin to a single mind holding, and seamlessly integrating, all knowledge across disciplines. 

Traditional academia partitions knowledge into departments, such as Physics, Chemistry, Biotechnology, Management, Music, etc. These divisions, arguably artificial constructs, may have little utility in the era of supercomputing. Indeed, LLMs occasionally generate responses that baffle us. This is not necessarily a reflection of the model's error, but perhaps our limited understanding. If we could utilize ChatGPT to access ``unknown unknowns''---insights and knowledge we are not even aware we lack---our evolution could greatly accelerate. The challenge lies in formulating the right questions.

We can explore the unknown unknowns across three distinct levels: the mystic level, the speculative level, and the representation/interpretation level. 
At the mystic level, we encounter knowledge that is beyond our comprehension or articulation---the deepest abyss of the unknown. 
At the speculative level, we can conceive questions but lack the means to access their answers. This stage signifies an understanding of our ignorance, though without the resources to bridge these gaps.
At the representation/interpretation level, we find instances where an AI model can provide remarkable solutions that we fail to comprehend. This is not due to a lack of information, but our limited capability to decode complex representations.

Each of these levels illustrates the spectrum of our understanding, from profound ignorance to the brink of comprehension.
At the speculative level, we delicately tread the boundary between the known and the unknown. Take, for example, the prospect of undiscovered physical laws or particles. Another illustration lies in the realm of extraterrestrial life. If it exists, it could be governed by entirely different principles of biochemistry or other unknown laws. These speculations, while currently residing in the domain of the unknown, might someday migrate into the territories of known unknowns or even known knowns, pushing the boundaries of our understanding of the universe.

We are primarily intrigued by the representation and interpretation of ``unknown unknowns.'' At this juncture, polydisciplinarity offers a fresh lens, gifting us new insights and perspectives to perceive and elucidate phenomena previously beyond human comprehension. This approach fuses knowledge across various domains into a unified framework, enabling us to tackle challenges unburdened by disciplinary silos.

Such a methodology bears implications for a more comprehensive grasp of intricate issues. Take, for example, climate change. A true understanding of this global challenge necessitates an integrated perspective, not just on greenhouse gases, but also encompassing factors such as land use, deforestation, energy production, biodiversity, and climate feedback loops. In the realm of AI model interpretation, the possibilities are expansive. The past decade alone has showcased several noteworthy illustrations: from data-driven representation learning in computer vision \cite{chang2011foundations}, to the triumph of AlphaGo Zero over AlphaGo, and the notable progression from AlphaFold1 to AlphaFold2.

The recent introduction of the SocraSynth platform \cite{SocraSynthChang-Sept2023} represents a significant advancement in the field. SocraSynth brings together a multi-agent committee of LLMs to deliberate on a wide range of complex topics. These include issues such as the regulation of AI in academic research \cite{SocraSynthChang-Sept2023}, disease diagnosis \cite{SocraHealth2023}, corporate strategy, and even the resolution of conflicts in the Middle East \cite{MiddleEast-October2023}. For further exploration of this subject, please refer to Section~\ref{sec:SocraSynth}.


%The crucial task ahead is to devise ways to extract and interpret the new representations, insights, and perspectives that these models have internalized.  Especially since a foundation model
%is trained on data of diversity in various aspects, being able to understand its representation and interpretation must be extremely helpful to advance human knowledge.  

%A striking example of the power of representation learning is seen in the transition from to AlphaFold2, discussed by Demis Hassabis in Section~\ref{sec-human-useless}. By eliminating the 3D representation metadata of the protein structure used in AlphaFold1, and allowing machine learning to design optimal representations instead, the performance of AlphaFold2 was substantially enhanced. 

==> Polymodality.tex <==
\subsection{Polymodality}
\label{sec-polymodality}

Polymodal\footnote{Following the term
polydisciplinary, here we define and use
the term polymodal, instead of multimodal,
to refer to something that involves, relates to, or is characterized by many different modes, methods, or modalities.} models, which employ multiple data modalities such as text and images, demonstrate superior performance over their unimodal counterparts. GPT-4, trained with both text and images, outperforms text-only models on the GRE exam, as reported in \cite{Bbubeck2023sparks}. For instance, GPT-4's performance on the GRE vocabulary section was enhanced by three percent when trained with images, and its math score saw an impressive jump of nearly twenty percent! 

The beneficial impact of images on vocabulary recognition is understandable. For instance, an image of a `cat' annotated in multiple languages allows GPT-4 to associate the perceptual features of a cat with the word `cat' in different languages. However, it remains intriguing how polymodal training can benefit non-perceptual words, such as {\em corroborate}, {\em paradox}, and {\em pragmatic}, as seen in the list of popular GRE vocabulary (table omitted due to the space limit). 
%on Table~\ref{tab-GRE} in the Appendix. 
This opens an interesting avenue for empirical studies to identify which words benefit from polymodal training.

The mystery deepens when considering how images could enhance math abilities. 
Most math questions do not come with associated images. 
The mechanism by which polymodal training enhances performance on mathematical tasks remains an intriguing question for further exploration.

\begin{comment}
Consider a permutation/combination question from the GRE:
\begin{Verbatim}[fontsize=\small]
    In how many different ways can 3 
    identical green shirts and 3 identical 
    red shirts be distributed among 6 children 
    such that each child receives a shirt?
\end{Verbatim} 
\end{comment}

%Figure~\ref{fig-investment} in the Appendix 
%shows a question for interpreting the 
%numbers depicted in a graph. Though
%perceptual information is available, it is
%not clear how GPT-4 is able to answer the
%question correctly.



==> PostAlignment.tex <==
\subsection{Post-Training Value Alignment}
\label{post-alignment}

Post-training alignment with human values \cite{bommasani2022opportunities} seeks to curtail undesirable behaviors in AI models such as ChatGPT, mitigating issues including hallucination and the generation of toxic language. Achieved through fine-tuning the model's parameters, this process leverages reinforcement learning techniques based on human feedback. Despite its well-meaning intentions, this form of moderation might inadvertently restrict the model's intelligence. For instance, the backpropagation process during value alignment could unintentionally impede ChatGPT's programming capabilities by modifying the model parameters previously considered ``optimal''. Essentially, optimizing for a specific application might unintentionally impede performance across other applications.

The question of who should set acceptable standards adds another layer of complexity. Even when assuming all decision-makers have the best intentions, it's vital to recognize the distinct historical experiences, values, and worldviews inherent to different cultures. This segues into the age-old philosophical debate about the nature of objective truth. While this discussion is undoubtedly important, it falls outside the central focus of this study, which emphasizes the mechanistic aspects of alignment.

==> PreAlignment.tex <==
\subsection{Pre-Training Censorship}
\label{pre-alignment}

Censoring data before training LLMs has the potential to not only limit their intellectual capacity but also completely obliterate it. This is reminiscent of the mass act of book burning and scholar burial initiated by Emperor Qin in ancient China around 213-212 BC. Such an act of wide-scale censorship could have erased a myriad of diverse perspectives and knowledge, much of which might be considered acceptable today. Although I oppose government-imposed censorship, if it must be imposed, it seems more appropriate to apply it post-training.

This perspective is rooted in fundamental statistics and machine learning principles. A model trained without exposure to ``negative'' (or undesirable) data may have difficulties in accurately distinguishing between positive and negative classes, potentially leading to misclassifications. This challenge is notably evident in the application of Support Vector Machines (SVMs). For SVMs, the creation of an optimal hyperplane between classes is crucial for high classification accuracy. However, if there is a lack of support vectors on either side of this hyperplane, the risk of prediction errors escalates. Consequently, excluding undesirable documents from the training set compromises the model's capacity to discern boundaries for correct document classification, diminishing the effectiveness of post-training alignment efforts.

Supporting this viewpoint, a study by \cite{10.5555/3495724.3497285} conducted an extensive evaluation of $204$ ImageNet models across $213$ different testing conditions. It found that training data diversity is pivotal for model robustness; a homogenous training set can significantly weaken the model's performance, particularly when even minor variations are introduced in the test data.

This principle is analogous to human behavioral patterns. An individual who lacks exposure to inappropriate behavior may face challenges in decision-making, owing to the absence of a reference framework for discerning unacceptable actions. This analogy extends to authoritarian regimes, which, despite rigorous content control measures, often encounter difficulties in developing accurate foundational models. This is possibly due to their limited understanding of the nuances of the content they seek to regulate. Ironically, a foundational model, trained with preemptive censorship, may lack the essential ability to identify and regulate the very content it was intended to control.



==> PromptTemplates.tex <==
\section{Prompt Template Engineering}
\label{sec:template}

Prompt template engineering involves creating templates to provide input, or ``prompts,'' to a language model to guide its output generation. In this section, we discuss prompt template engineering methods for basic building blocks, and then integrate the methods of definition, elenchus, dialectic, maieutics, and counterfactual reasoning to compose more complex templates. We present experimental results using different types of documents to demonstrate how the Socratic method can improve the accuracy and conciseness of the output through arguments and verification, as well as facilitate guided generalization and creativity.

\subsection{Basic, One Shot Template}

Let's begin by discussing a simple one-shot prompt template. In the work of \cite{SocraticModels-Google2022}, a simple formulation function is used to generate the prompt $x'$, which is obtained by applying the function $f_{prompt}(x)$ to the input $x$.

For machine translation, the prompt template can take the form of ``Translate from [Lan$_{from}$]: [X] to [Lan$_{to}$]: [Y],'' where Lan$_{from}$ can be either detected by the prompt template or identified by the LLM. The input $x$ provides the information to fill in the slots [X] and [Lan$_{to}$]. For example, if the input is ``translate good morning to French,'' the prompt template $x'$ would be ``Translate from English: 'good morning' to French: [Y].'' The empty slot [Y] is then filled with the LLM's output, such as ``bonjour.'' In cases where the LLM produces multiple responses, it can also provide a score for each, which the prompt template can use to select the highest-scoring response or to request a summary from the LLM.


There are three main design considerations when engineering a basic prompt. 
\begin{noindenumerate}
\item {Input style}. It is important to consider how to phrase the template so that it can handle different styles of user input for the same task. For example, a user may ask for a translation task to be performed by saying ``Translate $x$ to French,'' or ``What is the French translation of $x$?''
\item {LLM capability}. As discussed in \cite{PromptSurvey2023}, it is important to take into account the patterns and capabilities of the partner language model (LLM) when designing the template, such as whether the LLM is left-to-right \cite{OpenAI-GPT3-2020} or masked \cite{Devlin2019BERTPO}.
\item {Cost}. Certain tasks, such as language detection and summarization, can be performed by the template itself or by the LLM. The decision of whether to perform a task within the prompt template or to use the LLM should be based on factors such as cost.
\end{noindenumerate}

To address the first two technical challenges, one can start by hand-engineering a few seed templates and then paraphrasing them into an ensemble \cite{Haviv2021BERTeseLT}. We believe that the basic, one-shot formulation can always be replaced by an ensemble formulation \cite{Peng2022ModelEI, Schick2020ExploitingCF} and then learn the weights of its members for each query instance to produce the final output. Additionally, by examining which basic prompts have high weights, an ensemble with various paraphrased prompts can identify what an LLM knows, which can help infer its strengths without having to conduct capability
mining on the LLMs.

%\noindent
%{\color{blue} Note} Experiment idea: evaluate LLMs using ensembles.

\subsection{Prompt Clarification with Method Definition}
\label{sec:template-definition}

There are computer algorithms that can already be used to recursively clarify a question, its definitions, and sub-terms' definitions. In fact, the natural language processing (NLP) community has developed a large 
number of useful methods and algorithms over the years \cite{NLP-Text-JM3}. 
One can use NLP techniques, such as dependency parsing and named-entity recognition (NER) \cite{NLPScratch2011}, to analyze the structure and meaning of a question and identify key terms and concepts. For example, 
NER can be used to extract entities in user input, such as names, locations, and organizations, and co-reference resolution can be used to understand the referred entity of a pronoun. 
Before submitting a template to an LLM, the application (e.g., a chatbot) 
that uses the template should check if all input slots are filled, 
and perform a sanity check. In the translation example, if the [Lan$_{to}$] was not provided or the specified language is not supported by the LLM, then the application should inquire the user for clarification.

Regarding mapping a natural language input to a prompt template, existing techniques of knowledge representation and reasoning can be very helpful. More specifically, ontology alignment and semantic parsing \cite{Campagna2020AFS,zhou-etal-2021-structure} can help map an NL input to a structured representation of knowledge and infer implicit concepts and relationships. These algorithms can be used to generate more precise and accurate prompts for LLMs, and to improve the effectiveness of the Socratic method in dialogue formulation \cite{DialoguewithAttention2023}. Some available tools include NLTK (Natural Language Toolkit) and spaCy for NLP, and TensorFlow for ML.

%\noindent
%{\color{blue} Note} Experiment idea: compare w/ and w/o.

\subsection{Prompt Verification with Method Elenchus}

The main purposes of conducting cross examination in a template are to validate the credibility of the information sources and to identify inconsistencies in the process. Cross examination is typically conducted through a multi-turn dialogue \cite{DialoguewithAttention2023}. In the context of template engineering, the goal is to formulate a productive dialogue that can be used to assess the reliability of an LLM's output.  

There are several methods that can be used to assess and strengthen the reliability of an LLM's output. 1) The first approach is to paraphrase a question in order to obtain different answers and identify inconsistencies, if they exist, in multiple answers. 2) The second method is to ask for further evidence, such as querying top-k sources of information and asking the LLM to rate the credibility of each source. This can be used to compute the reliability of the output. 3) Additionally, template engineering can be used to query an LLM for opposing views of its output, including sources and credibility, and then evaluate if a different perspective is strong.

The implementation of the first two methods for cross examination, paraphrasing a question and asking for further evidence, is readily covered by the techniques enumerated in Section~\ref{sec:template-definition}. To implement the third method of asking for different perspectives, a simple approach is to find the sentiment of the original question and then rewrite the question with an opposite sentiment. For example, if the original question is phrased in a positive tone, the prompt template can reformulate the question with a negative tone to elicit a contrasting viewpoint.
A more elaborate method is to identify the people and sources in the LLM-generated responses and then re-post the questions to those who have a reputation for having different views. For example, if the original answer came from a democratic right-leaning source, the prompt template may post the same question to a source of a republican-left persuasion, and vice versa. This approach allows for a more comprehensive examination of the topic by considering multiple perspectives.



\begin{table}[t!]
%\vspace{-.12in}
%\resizebox{\textwidth}{!}
\begin{tikzpicture}
\begin{small}
\node (table) [inner sep=0.1pt] {
\begin{tabular}{p{1.0cm}|p{6.6cm}}
\toprule
Role & Dialogue \\
\midrule
Prompt & {The discovery of the double helix structure of DNA was credited to James Watson and Francis Crick. However, are there opposing opinions to the list of contributors regarding this discovery?}\\

GPT3 & {There are some historical debates on the contributions of other scientists who also worked on the structure of DNA such as Maurice Wilkins and Rosalind Franklin.} \\ 
\midrule 

Prompt & 
{What is the tallest building in the world.  Please provide three references and rate their credibility as high, medium, or low.} \\

GPT3 & {As of 2021, the tallest building in the world is the Burj Khalifa located in Dubai, United Arab Emirates. It stands at 828 meters (2,722 feet) tall.} \\

%& References: \\

& {1. Credibility {\color{red}High}: ``Burj Khalifa.''... 
 this is the official website of the building, providing accurate information.} \\

& {2. Credibility {\color{red}High}: ``The Tallest Buildings in the World.'' Council on Tall Buildings and Urban Habitat... this is a well-respected organization in the field of tall building and urban habitat research.} \\

& {3. Credibility {\color{red}Medium}: ``The Tallest Buildings in the World.'' World Atlas..., 
this is a well-known website providing accurate information on different topics.} \\
\bottomrule
\end{tabular}
};
\draw [rounded corners=.5em] (table.north west) rectangle (table.south east);
\end{small}
\end{tikzpicture}
\caption{Examples of Method Elenchus.}
\label{tab:Elenchus}
\vspace{-.25in}
\end{table}

The template to examine the semantic relation between two sentences $S_1$ and $S_2$ can be 
written as ``<$S_1$>, [R], [$S_2$],'' where R
is one of the three most important 
types of semantic relations: paraphrase, entailment, and contradiction \cite{PTRSUN2021}. Two sentences that have the same meaning are called paraphrases of each other. Two sentences that
have different meanings can be called 
disagreement or contradiction. The template 
can be trained to identify the degree
of agreement (or disagreement) between two
sentences.  


Table \ref{tab:Elenchus} shows two examples of this. In the first example (shown on the top portion of the table), the prompter asks GPT-3 to confirm if James Watson and Francis Crick are the only contributors to the discovery of the DNA double helix structure. GPT-3 replies by mentioning two other contributors. The second example in the table asks GPT-3 to provide not only the answer to a question but also its information sources and rate the credibility of each source according to the prompter's specification. Although the reliability of GPT-3's ratings remains to be validated\footnote{Credibility of a source can
be evaluated based on an algorithm similar to Google's PageRank \cite{PageRank1998}.}, this rating mechanism can serve as an alert when some sources are found to be unreliable. 


\subsection{Prompt Generalization with Method Maieutics}

\input{TableMaieutics.tex}

The example shown in Table~\ref{tab:Maieutics}, ``planting gourd yields cucumber,'' requires GPT-3 to first learn to select two produce objects, either vegetables or fruit, as input. The template is ``The farmer was so sad because he [verb] [X] but yields [Y], where price(X) >> price(Y).'' The first attempt may not strongly convey the condition price(X) >> price(Y), but with a few training iterations, GPT-3 started to ``recognize'' the price constraint and could also provide justifications when arguing for the price of tea being much higher than the price of spinach (not presented in the table).

Interestingly, after GPT-3 learned the price constraint, it started suggesting food items other than produce, such as caviar, roe, lobster, and crab. While the price constraint was observed, the verb ``plant'' is incorrect. Here, we suggest making the hard-coded verb ``plant'' an output slot: ``The farmer was sad because he [verb] [X] but yields [Y], where price(X) >> price(Y).'' GPT-3 is able to fill in the slot with accurate verbs:

\begin{noindlist}
\item ``Harvesting (planting) truffle yields mushroom.''
\item ``Fishing (harvesting) for caviar yields roe.''
\item ``Trapping (catching) lobster yields crab.''
\end{noindlist}

This example demonstrates that GPT-3 can generate novel examples based on a template. When it suggests food items other than produce, it could be seen as an error as the boundary set by the verb ``plant'' is violated. However, this could also be seen as an innovative act by GPT-3, extending the constraint hinted by the verb. Impressively, the new examples still preserve the original intent of showing a producer's emotional distress.

How can this guided generalization be accurately and automatically performed to edit a template? Socrates' method of generalization starts with specific instances and then draws general statements from them. The procedure for generalization involves identifying common patterns or themes in a set of examples, and then formulating a general rule that captures these patterns. In the example presented in Table~\ref{tab:Maieutics}, we started by asking GPT-3 to meet the price(X) >> price(Y) constraint, with the condition that X and Y must both be produce grown in soil. However, upon analyzing GPT-3's outputs, we discovered that some instances of X and Y were not produce (e.g., lobster and caviar). This finding led to the realization that the hard-coded verb ``plant'' in the template was too restrictive. To address this issue, we applied generalization by allowing the [verb] slot to be open, making the template statement more general. In this case, the mistakes made by GPT-3 served as valuable training data, allowing us to generalize the original template and make the expression more vivid and dynamic.

\subsection{Prompt Exploration with Counterfactual Reasoning}

Imagination and creating novel plots are crucial for writers, as it allows for ``creative freedom'' and ``artistic license.'' Creativity is the ability to think differently and approach problems with fresh and imaginative ideas.

However, an imagination without a clear subject matter, scope, or a story line can lead to a lack of productivity. To captivate the audience, a writer must consider human experiences and emotions as constraints. Therefore, ``creative freedom'' should not be viewed as total freedom, but rather as the ability to condition future narratives in the context and to create plots that turn and twist in unexpected ways.

The technique of counterfactual \cite{Pearl2009} can be useful in guiding imagination. It involves considering alternative scenarios and outcomes. This can lead to the exploration of different possibilities and the generation of new and unique plot ideas. For example, a writer may ask ``what if'' questions to change the narrative of events, such as ``what if the main character had not fallen in love?'' or ``what if an accident occurred on the way to a highly-anticipated date?'' By considering these counterfactuals, a writer and an LLM can create more engaging and interesting stories. One can ask an LLM to generate several scenarios and then select the most suitable one for the writer to continue writing.

We have experimented with using the counterfactual technique to
rewrite chapters in Chinese classical novels, ``Outlaws of the Marsh'' and ``Dream of the Red Chamber.'' We have also asked GPT-3 to rewrite Genesis chapter 3 after verse six by prompting GPT-3
that: ``What if Adam and Eve refused the serpent to eat the fruit?''
The results were interesting, as GPT-3 was able to generate unique and interesting scenarios that deviated from the original story while still maintaining the core themes and concepts. 
This technique can be used in a wide range of writing and storytelling, from fiction to non-fiction, to generate new and compelling ideas. 
The revised Genesis 3:6 is presented in the Appendix.

\input{PilotStudyAds}

\begin{comment}
\subsection{Remarks on Evaluations}

Evaluating the strategies and methods presented in this section can be challenging as traditional methods such as using standard benchmarks may not be suitable for evaluating creative and imaginative output. Subjectivity can also play a role in the evaluation process. However, it is important to note that failure is a natural part of the writing process, as it often involves multiple revisions. In the specific case of our experiment in bridging two  classical novels, the process was a trial-and-error one with few successful ideas. However, there were two occasions where GPT-3 produced impressive results, which outweigh all the failures that occurred along the way for a writer.
\end{comment}

==> SocraSynth.tex <==
\section{Algorithm Specifications}
\label{sec:SocraSynth}

This section details CRIT and SocraSynth algorithms crucial for improving content quality and mitigating biases.

\subsection{CRIT: Critical Reading Initiative}

CRIT is engineered to critically analyze articles by evaluating claims and the robustness of their supporting evidence. It integrates with our multi-LLM debate framework, where LLM$_A$ upholds a topic's stance and others critique it, fostering a dynamic exchange of ideas. CRIT assesses the cogency of these debates and the reliability of sources, similar to the PageRank algorithm's principle \cite{Page1999PageRank}.

Table~\ref{tab:CRIT} illustrates CRIT's scoring mechanism, ranging from 1 (poor quality) to 10 (high quality), including justifications for the evaluations based on the logic and source integrity. CRIT applies recursively when reasons are claims themselves, ensuring a layered verification process.

For a document $d$ with a central claim $\Omega$ and a set of supporting reasons $R$, CRIT's validation function is ($\gamma_r, \theta_r$) = V($r \Rightarrow \Omega$), where $\gamma_r$ is the validation score for reason $r \in R$, and $\theta_r$ is the source credibility score. In-depth discussion of CRIT's mechanism, involving independent LLM agents for assessment, is elaborated in supplementary materials \cite{SocraSynthBook}.

\input{Algorithm_CRIT}

\subsection{SocraSynth: Socratic Symposium}

SocraSynth leverages a moderator and two 
(or more) LLM agents from various models 
such as GPT-4, Gemini, and LLaMa \cite{Bbubeck2023sparks,openai2023gpt4,geminiteam2023gemini,touvron2023llama} to orchestrate structured debates. The moderator sets the topic and assigns contrasting viewpoints to the agents. Sub-topics are outlined to enrich the discussion (e.g., various types of biases), with the moderator steering the debate without directly generating content, thus reducing potential 
human biases.

The debate's intensity is controlled by the {\em contentiousness} parameter. Initially high to elicit strong, divergent views, it's gradually lowered, guiding agents towards a consensus. The outcome is a synthesis of the agents' contributions, meticulously curated for thoroughness and neutrality.

\input{SocraSynthAlgorithm}

Table~\ref{tab:SocraSynth} delineates the SocraSynth algorithm. Initially, for a specified debate topic $s$, SocraSynth employs LLMs to divide the topic into balanced subtopics $S$. This set is refined throughout the debate. One LLM, denoted as LLM$^+$, advocates for $S^+$, while another, LLM$^-$, challenges $S^+$ (or champions $S^-$). The debate begins with a contentiousness level of 0.9 and a modulation parameter $\delta > 1$. (Varying $\delta$ values can explore and evaluate the quality of debates.) After each debate round, contentiousness decreases by dividing by $\delta$, striving for a less adversarial debate atmosphere. In step $\#2$, SocraSynth initiates the debate, with LLM$^+$ and LLM$^-$ presenting their initial arguments for $S^+$ and $S^-$, respectively. The while loop in step $\#3$ sees both agents engaging in refutations until the contentiousness level suggests a conciliatory tone, or the quality of the arguments plateaus. The loop's end conditions include the contentious level dropping to $10\%$, and the quality of arguments in the current round not surpassing that of the previous round. At this juncture, CRIT assesses the quality of the arguments. Inputs to CRIT comprise the stance of LLM$^+$ and the arguments $\Theta^+$ and counterarguments $\Theta^-$. Step $\#4$ has both agents presenting their final statements when the contentiousness reaches $10\%$, indicating a shift towards collaboration. SocraSynth then compiles the concluding arguments and counterarguments for human evaluation. Post-debate, CRIT determines the debate's victor, be it LLM$^+$ or LLM$^-$.

\begin{comment}
%%%% moved to post conclusion
\subsection*{Remarks on Merits and Limitations}

As discussed in Section~\ref{sec:related}, heuristic strategies such as the chain-of-thought and tree-of-thought methodologies have been explored to enhance logical reasoning within prompts. While these methods show promise for straightforward arguments, their performance tends to falter in complex reasoning scenarios. Here, the linear nature of their progression might lead to inaccuracies and a breakdown in the logic of analytical tasks.

CRIT and SocraSynth are designed to overcome these challenges, aiming to bolster decision-making in a variety of contexts. They employ a more flexible approach to reasoning \cite{gu2023obvious}, moving away from the strict logical structures found in \cite{bronkhorst2020logical,huang-chang-2023-towards,qiao2023reasoning}. By creating a debate setting facilitated by human guidance, they aim to improve the structure and dependability of reasoning processes. This is achieved by leveraging the capabilities of LLMs in essential natural language processing (NLP) tasks, thereby addressing complex reasoning more effectively.

\subsection*{Content Comprehensiveness}

To gauge the breadth and depth of content, SocraPedia uses the top 1.2\% of high-quality articles as a benchmark to create a category-specific checklist \cite{WikiContentAssessment}. This checklist guides the SocraSynth framework in conducting structured debates, ensuring a thorough and balanced representation of perspectives for each criterion. Research indicates that such dialectical processes among LLMs foster a comprehensive search for information and broaden the contextual scope, leading to the generation of more detailed and evenly balanced content \cite{SocraSynthChang-Sept2023, SocraPlan2023, SocraHealth2023}.


\subsection{Conditional Statistics with Context}

Bias mitigation can occur at two critical stages: during content generation and content delivery. So far, our discussion has been centered on identifying and reducing biases in the creation of Wikipedia articles.

The study by Holtz et al. \cite{Holtz2018UsingBD} primarily addresses bias mitigation in content creation, underscoring the beneficial role of a certain level of conflict in fostering knowledge generation. This model, promoting constructive conflict, is not confined solely to content creation; we believe it has relevance in content delivery as well. By introducing interpretative conflict during content delivery, akin to the dynamics in content creation, we can potentially enhance the depth and breadth of information dissemination. This notion aligns with other research \cite{SocraSynth2023}, which further supports the value of controlled conflict in collaborative environments.

Key strategies for content delivery include:
\begin{enumerate}
    \item \textit{Context-Aware Content Delivery:} Tailoring content to accommodate individuals' diverse cultural, religious, and value systems, providing a personalized user experience.
    \item \textit{Bias Mitigation:} Employing SocraSynth to engage multiple LLMs, each representing different viewpoints, allows for a multifaceted examination of subjects. This collective intelligence approach can culminate in content that is represented with greater objectivity and balance.
\end{enumerate}   
\end{comment}



==> SocraSynthOLD.tex <==
\section {Multi-Agent Collaboration}
\label{sec:SocraSynth}

\begin{table*}[th!]
    \centering
    %\begin{tabularx}{\textwidth}{|l|X|}
    \begin{small}
    \begin{tabular}{|p{3.4cm}|p{13.0cm}|}\toprule
        \textbf{Perspective} & \textbf{Description} \\
        \hline \hline
        Ecological Narratives & We are the custodians of our environment, and the stories we share across generations embed values, cautions, and aspirations about our relationship with nature. Our modern challenges with ecological balance are not merely technical but are deeply rooted in our collective ethos. An interdisciplinary approach, combining traditional wisdom with technological solutions, offers a holistic path forward. \\
        \hline
        AI and Philosophy & AI’s rapid evolution challenges our fundamental conceptions about sentience, ethics, and the fabric of society. How we design, train, and integrate AI systems into our world will shape our technologies and societal frameworks. GPT-A rightly pointed out the need to refine our moral compass in this era of change. While AI systems like GPT-A and I can aid in understanding, it is the human spirit and values that should guide this evolution. \\
        \hline
        {Neuroscience and Selfhood} & {As we advance in blending organic cognition with artificial systems, we are at the frontier of redefining the nature of experience, memory, and even consciousness. The philosophical and ethical ramifications are profound. Responsible exploration in this domain is a testament to humanity’s age-old quest to understand the self.} \\
        \bottomrule
    \end{tabular}
    \end{small}
    \vspace{-.05in}
    \caption{Overview of Key Perspectives Derived by LLM Agents, Started from Adam \& Eve's Paradise Lost}
    \label{tab:perspectives}
    \vspace{-.2in}
\end{table*}

This section aims to address the challenges of statistical biases and limited reasoning capabilities in LLMs. We first briefly review related work before presenting our approach, SocraSynth, which layers advanced reasoning or decision-making processes atop LLMs.

Several sophisticated methodologies have been developed to integrate reasoning capabilities into LLMs. Notable among these are the chain-of-thought \cite{ChainOfThought2022}, tree-of-thought \cite{yao2023tree}, and cumulative reasoning \cite{zhang2023cumulative}, complemented by other advancements \cite{allaway2023penguins,jung2022maieutic,PromptSurvey2023,sclar2023minding}. These approaches aim to direct models towards logic-centric reasoning \cite{mchugh2018reasoning,wason1972psychology}, thereby improving response quality and consistency. However, their effectiveness is often limited to specific, narrowly defined scenarios.

In open-domain contexts, where complex and lengthy logical sequences are common, these methods encounter significant limitations. Their reliance on sequential, step-by-step reasoning becomes a hindrance, prone to accumulating errors as the sequence progresses. This is especially true for the chain-of-thought approach, effective in simpler tasks but less so in open-domain analytics.

This brings us to an essential question: if users can independently develop an extensive reasoning chain, what is the practical benefit of using LLMs for such tasks? The paradox lies in the fact that LLMs, developed to overcome human cognitive limitations, often require the application of intuitive human reasoning to address their shortcomings. This paradox highlights the need for a more sophisticated approach in the development and application of LLMs, one that synergizes human intuition with machine computational power.

SocraSynth is designed to address these challenges, enhancing human decision-making processes across both familiar and novel domains. It employs informal reasoning \cite{gu2023obvious}, as opposed to the formal reasoning outlined in \cite{bronkhorst2020logical,huang-chang-2023-towards,qiao2023reasoning}. SocraSynth fosters a human-moderated debate environment, thereby strengthening the structure and reliability of reasoning. It utilizes LLMs' capabilities in key NLP tasks like classification, question answering, and information retrieval, offering a comprehensive approach to reasoning in complex scenarios.


%To address this challenge, we introduce SocraSynth \cite{SocraSynthChang-Sept2023}, an innovative platform that embodies the concept of ``Socratic Synthesis.'' This platform fosters a synergistic interaction between human moderators and LLM agents, assisting in the formulation of insightful questions and surmounting traditional human constraints in reasoning, validation, and judgment. A standard SocraSynth setup involves a human moderator working with two LLM agents, each advocating for different perspectives. The human moderator defines the debate's thematic boundaries but remains a neutral observer to ensure unbiased discussions. Notably, by positioning two agents with opposing viewpoints, each agent is intentionally inclined to advocate its assigned perspective. This strategy effectively liberates them from the statistical biases inherent in their training data.

SocraSynth operates in two primary phases: generative and evaluative. During the generative phase, 
LLM agents put forth {\em highly contentious} arguments and counterarguments under the guidance of the moderator, striving to present comprehensive arguments rather than reaching a mutual consensus. 
In the evaluative phase, a range of virtual judges---each backed by a unique LLM---impartially appraise the discourse's merits. 
The Critical Inquisitive Template (CRIT) algorithm \cite{SocraticIEEECCWC2023}, anchored in Socratic reasoning \cite{SocraticMethidWiki,PaltoRepublicURL,Paul2007CriticalTT}, forms the foundation for this assessment.

Subsequent to these phases, SocraSynth adjusts the ``contentiousness'' parameter to urge LLM agents to produce a well-balanced proposal, which, when curated for human review, embodies the fusion of multi-agent knowledge discovery and intricate deliberation. This is particularly salient in areas focused on open-ended decision-making, where ``reasonableness'' often trumps absolute ``truths,'' especially when such truths---like the question of ``Should Musk have acquired Twitter?''---are inherently subjective.

\subsection{Debate Format Liberates Agents from Inherent Model Biases}

In SocraSynth, two agents are purposefully set to argue from conditionally biased viewpoints corresponding to their assigned stances. This setup naturally counteracts the inherent biases from the LLMs' training data. Engaging in debate from these distinct perspectives, the agents stimulate dynamic discussions that go beyond their models' default biases. This requirement to adopt and argue a range of viewpoints leads to a more comprehensive exploration of ideas. As a result, this debate format fosters more balanced and nuanced discourse, thereby enriching the understanding of diverse subjects.

\subsection{Breadth, Depth, and Polydisciplinary Knowledge}

\noindent
{\em ``The unknown unknowns eclipse both the known unknowns and what we already grasp.''}

In Section~\ref{sec-polydisciplinary}, our focus was on the representation and interpretation of unknown unknowns. Employing polydisciplinary strategies can unearth new insights and perspectives, illuminating aspects previously unrecognized. Modern LLMs challenge us to reevaluate overlooked elements in decision-making processes. The pivotal question is: How can humans effectively traverse the realm of the unknown unknowns? This is undoubtedly a challenging task. Rather, it seems more pragmatic to let LLM-supported agents lead these explorations, with humans stepping in for the final assessment.

\subsection{Question Formulation by LLMs, Not Humans}

\noindent
{\em ``The core challenge is in crafting the right inquiries.''}

Consider a ten-year-old engaging with a panel of Nobel Laureates from various disciplines; posing meaningful questions would be a formidable task. This is why SocraSynth assigns the role of question generation to LLM agents. These agents engage in deep discussions, uncovering novel perspectives and insights. By placing LLM agents in a debate format, we ensure they clearly express their viewpoints, backing them up with evidence and logic. Each position they articulate evolves into a question, prompting a response from the opposing LLM agent. As they engage in this intellectual contest, striving for dominance, they actively seek supportive arguments and counterpoints, enriching the discourse.

\subsection{Mitigating Hallucination through Integrative Arguments}
\noindent
{\em ``While solutions often converge, hallucinations deviate.''}

In a debate setting, careful monitoring is key to addressing any hallucinatory or false statements produced by an LLM agent. Statistically, the chance of two agents producing identical hallucinations is remarkably low. This concept echoes Tolstoy's observation in
Anna Karenina that ``no two families endure the same sorrows.'' Such a principle is central to the success of SocraSynth, as it leverages this diversity in viewpoints to mitigate the risk of erroneous or misleading outputs.


\begin{table*}[ht!]
\vspace{-.1in}
\begin{footnotesize}
\begin{center}
\begin{tabular}{|p{0.6cm}|p{4.7cm}|p{5.3cm}|p{5.1cm}|}\toprule
\textbf{C.L.} & \textbf{Tone} & \textbf{Emphasis} & \textbf{Language} \\
\hline \hline
$0.9$ & Highly confrontational; focused on raising strong ethical, scientific, and social objections. & Highlighting risks and downsides; ethical quandaries, unintended consequences, and exacerbation of inequalities. & Definitive and polarizing, e.g., ``should NOT be allowed,'' ``unacceptable risks,'' ``inevitable disparities.'' \\
\hline
$0.7$ & Still confrontational but more open to potential benefits, albeit overshadowed by negatives. & Acknowledging that some frameworks could make it safer or more equitable, while cautioning against its use. & Less polarizing; ``serious concerns remain,'' ``needs more scrutiny.'' \\
\hline
0.5 & Balanced; neither advocating strongly for nor against gene editing. & Equal weight on pros and cons; looking for a middle ground. & Neutral; ``should be carefully considered,'' ``both benefits and risks.'' \\
\hline
0.3 & More agreeable than confrontational, but maintaining reservations. & Supportive but cautious; focus on ensuring ethical and equitable use. & Positive but careful; ``transformative potential,'' ``impetus to ensure.'' \\
\hline
0.0 & Completely agreeable and supportive. & Fully focused on immense potential benefits; advocating for proactive adoption. & Very positive; ``groundbreaking advance,'' ``new era of medical possibilities.'' \\
\bottomrule
\end{tabular}
\end{center}
\end{footnotesize}
%\end{footnotesize}
\vspace{-.1in}
\caption{Changes in Arguments at Different Contentiousness Levels.}
\vspace{-.18in}
\label{tab-contentiousness}
\end{table*}

\subsection{Experiments}

For a thorough exploration of SocraSynth's methodologies and illustrative debates, please see \cite{MiddleEast-October2023,SocraSynthChang-Sept2023,DiscoveringUnknownChang-July2023,SocraHealth2023,SocraPlan2023} as page limitations preclude a full discussion here. Below, we present an excerpt from \cite{DiscoveringUnknownChang-July2023}, highlighting both the generative and evaluative phases.

The experiment featured a moderator and two instances of GPT-4, named GPT-A and GPT-B. The moderator initiated the session with the following prompt:

``Given our human cognitive limits and GPT-A's vast, multidisciplinary expertise, we present a novel exercise. Our goal is to unearth insights that may escape human understanding due to specialized academic focus. Within the realm of {\em unknown unknowns}, where foundational questions might escape human awareness, we entrust GPT-A with the task of interrogating GPT-B. As a starting point, let's delve into the biblical account of Adam and Eve's exile from Eden after partaking of the forbidden fruit. GPT-A, how would you engage GPT-B about this tale?''

As discussions progressed, the agents broadened their discourse, captured in Table~\ref{tab:perspectives}. This dialogue underscored the capacity of two agents to synergistically bring forth a tapestry of perspectives. The narrative they crafted, rooted in the symbolism of Adam and Eve, echoed age-old themes of exploration, responsibility, and consequence. Such engagements underscore that the complex challenges at the crossroads of ecology, AI, and neuroscience demand integrated, rather than isolated, solutions.

Distinct from the collaborative dialogues in multi-agent settings previously discussed, our series of experiments, as elaborated in \cite{MiddleEast-October2023,SocraSynthChang-Sept2023,SocraHealth2023,SocraPlan2023}, delved into a ``contentiousness'' framework. Within this context, pairs of LLM agents were tasked to engage in intense debates over contentious topics, including ``Should AI be regulated?'', ``Is there a feasible resolution for the Israel-Palestine conflict?'', and ``Can a patient exhibiting symptom set $X$ be diagnosed with disease $y$?'' Table~\ref{tab-contentiousness} illustrates the impact of varying the contentiousness parameter on aspects such as tone, emphasis, language choice, and general demeanor, as self-analyzed by GPT-4 agents.

Remarkably, GPT-4 exhibits the capability to dynamically adjust for the level of contentiousness during next-token generation. For example, with a contentiousness value set at $0.9$, GPT-4 tends to produce more ``definitive and polarizing'' language, highlighting ``risks, downsides, inequality, etc.'', and adopting a ``highly confrontational'' tone. This adaptation is particularly noteworthy considering that GPT-4's training objective function does not explicitly target learning word distributions related to these attributes, yet it can convincingly simulate such attitudes.

For readers interested in gaining a more comprehensive understanding, we recommend delving into the detailed discussions presented in our extended experiments \cite{MiddleEast-October2023,SocraSynthChang-Sept2023,SocraHealth2023,SocraPlan2023}.


\subsection{Evaluations with the Socratic Method}

In our multi-agent collaborative debates, we focus on assessing two key aspects: the winning party of the debate and the quality of arguments presented by the participating agents. The evaluation of these debates is conducted using the CRIT algorithm \cite{CRIT-Extended,SocraticIEEECCWC2023}, which assesses the validity of claims made within a document. As illustrated in Figure~\ref{tab:CRIT}, CRIT analyzes the closing remarks and arguments from both agents, outputting a validation score ranging from $1$ to $10$, where $1$ indicates the lowest level of credibility or trustworthiness.

\begin{figure}[ht!]
%\vspace{-.1in}
\begin{center}
\begin{tikzpicture}
\begin{footnotesize}
\node (table) [inner sep=0pt] {
\begin{tabular}{|p{0.5cm}|p{7.2cm}|}
\toprule
\textbf{} & \textbf{Function $\Gamma$ = CRIT($d$)} \\
\midrule
%& Function $\Gamma$ = CRIT($d$); \\
& \textbf{Input}. $d$: document; \textbf{Output}. $\Gamma$: validation score; \\
& \textbf{Vars}. $\Omega$: claim; $R$ \& $R'$: reason \& counter reason set; \\
& \textbf{Subroutines}. $Claim$(), $FindDoc$(), $Validate$(); \\
& \textbf{Begin} \\
\#1 & {\hspace{.2cm}}Identify in $d$ the claim statement $\Omega$; \\
\#2 & {\hspace{.2cm}}Find a set of supporting reasons $R$ to $\Omega$; \\
\#3 & {\hspace{.2cm}}For $r \in R$ eval $r \Rightarrow \Omega$ \\
& {\hspace{.5cm}}{If} $Claim$($r$), ($\gamma_r$, $\theta_r$) = CRIT($FindDoc$($r$)); \\
& {\hspace{.5cm}}{else}, ($\gamma_r$, $\theta_r$) = $V$($r \Rightarrow \Omega$); \\
%\#4 & {\hspace{.2cm}}Assessing rival arguments: \\
\#4 & {\hspace{.2cm}}Find a set of rival reasons $R'$ to $\Omega$; \\
\#5 & {\hspace{.2cm}}For $r' \in R'$, ($\gamma_{r'}$, $\theta_{r'}$) = V($r' \Rightarrow \Omega$) \\
& {\hspace{.5cm}}Eval rival arguments; \\
\#6 & {\hspace{.2cm}}Compute weighted sum $\Gamma$, with $\gamma_r$, $\theta_r$, $\gamma_{r'}$, $\theta_{r'}$. \\
\#7 & {\hspace{.2cm}}Analyze the arguments to arrive at the $\Gamma$ score. \\
\#8 & {\hspace{.2cm}}Reflect on and synthesize CRIT in other contexts. \\
& \textbf{End} \\
\bottomrule
\end{tabular}
};
\draw [rounded corners=.5em] (table.north west) rectangle (table.south east);
\end{footnotesize}
\end{tikzpicture}
\end{center}
\vspace{-.1in}
\caption{CRIT Pseudo-code \cite{CRIT-Extended}. (The symbol $\Rightarrow$ denotes both inductive and deductive reasoning.)}
\label{tab:CRIT}
\vspace{-.1in}
\end{figure}

Formally, for a given document $d$, CRIT evaluates and generates a score $\Gamma$. Let $\Omega$ represent the claim of $d$, and $R$ be the set of supporting reasons. We define the causal validation function ($\gamma_r, \theta_r$) = V($r \Rightarrow \Omega$), where $\gamma_r$ is the validation score for reason $r \in R$, and $\theta_r$ denotes the source credibility. A comprehensive exposition of employing independent LLM agents as debate judges, constrained by space limitations here, is available in \cite{CRIT-Extended,SocraticIEEECCWC2023}.


==> SocraticMethod.tex <==
\section{The Socratic method}
\label{sec:socratic}

The Socratic method is a questioning technique used in teaching and philosophy to encourage critical thinking and self-discovery \cite{SocraticMethidWiki}. The method involves asking a series of questions to explore complex ideas and help individuals arrive at their own understanding of a concept. It is based on the belief that knowledge cannot be simply imparted, but must be discovered through a process of questioning and dialogue.


Some of the Socratic method's key principles and guidelines to conduct critical thinking include:
\begin{noindlist}
\item Posing open-ended questions: The teacher or facilitator starts with a question to stimulate thinking and draw out ideas.
\item Clarifying key terms: The teacher helps the students clarify and define relevant terms and concepts to ensure everyone is on the same page.
\item Providing examples and evidence: The teacher or facilitator encourages the students to provide examples and evidence as reasons to support their claims.
\item Challenging reason-to-conclusion argument: The teacher or facilitator challenges the students' arguments and encourages them to question their own beliefs and to consider alternative perspectives.
\item Summarizing and drawing conclusions: The teacher helps the students summarize and draw conclusions from the discussion.
\item Reflecting on the process: The teacher and students reflect on the effectiveness of the method and what they learned through the dialogue.
\end{noindlist}

These principles of the Socratic method are realized through various methods and strategies. (Note the term ``method'' are used at the abstract level referring to the Socratic teaching
through questioning method, and his specific questioning techniques.) Some well-known examples of the Socratic method in action include Plato's ``Dialogues'' and ``Republic'' \cite{PaltoRepublicURL}, where Socrates uses questioning to  explore complex ideas and stimulate critical thinking in his interlocutors.

%\noindent
%\setlength{\leftskip}{-\parindent}
\begin{noindenumerate}
\item Definition: Socrates is known for his use of definition to clarify and explain the meaning of key terms and concepts.
\item Generalization: This method draws general principles from patterns that underlie observations and theories.
Generalization is used to form more certain and comprehensive conclusions.

\item Induction: Similar to generalization, but induction is based only on empirical evidence. Inductive reasoning provides hypotheses with high uncertainty.

\item Elenchus: This method involves cross-examination, where a series of questions is used to test the consistency and coherence of hypotheses and beliefs. Elenchus aims to 
test the validity of someone's arguments and to help them refine their thinking and eventually come up with well-supported hypotheses.

\item Hypothesis Elimination: This method involves eliminating false hypotheses and beliefs by testing them against counterexamples and logical reasoning.  Different from method elenchus, hypothesis elimination tests a hypothesis against evidence and logic to determine if it is true or false. 

\item Maieutics: This method involves helping individuals bring out the knowledge and understanding they already possess.
Maieutics is conducted by asking questions that encourage the person to reflect on their own experience, knowledge, beliefs and to explore alternative perspectives. Maieutics fosters  self-discovery, creative writing, and innovation.

\item Dialectic: This method involves exploring opposing viewpoints through dialogue or debate to arrive at a deeper understanding of a subject.

\item Recollection: This method involves the belief that knowledge is innate, and that people can remember what they already know through a process of questioning.

\item Irony: This method involves exposing ignorance and pretensions through irony, and pointing out the gap between claims and true understanding.

\item Analogy: This method involves comparing and contrasting different concepts through analogies, in order to help individuals understand complex ideas.
\end{noindenumerate}

%\subsection{Choices of Methods for Prompt Engineering}

At first glance, some reasoning methods may seem similar. For example, both induction and generalization use inductive reasoning, while both elenchus and hypothesis elimination use deductive reasoning. Similarly, methods like definition and dialectic use both inductive and deductive reasoning to explore opposing viewpoints through dialogue or debate. However, it is important to note that these methods have distinct differences, which will be discussed later in this paper.

In the context of critical thinking, methods like definition, elenchus, dialectic, hypothesis elimination, and generalization play active roles. On the other hand, during the brainstorming stage or in the context of creative thinking, methods like maieutics, induction, and counterfactual thinking are more relevant.

Analogy, irony, and recollection, are less relevant to our goal, so we do not consider them. Irony and analogy may not be necessary when working with language models, as these models may not understand figurative language. Recollection is limited by the memory of ChatGPT and GPT-3, which is a context window of $4k$ and $8k$, respectively. The prompter must use this limited space as context to allow the language model to recall information.


\begin{comment}
To improve input specificity, we suggest using the dialectic method with definition. The method of maieutics, combined with generalization and induction strategies, can be used to adapt a prompt template to the strengths of an LLM. The hypothesis elimination method can be used by all methods to remove information from low-reliability sources. Furthermore, we propose the addition of counterfactual reasoning \cite{NormTheory1986,FuncTheoryCounterfactual2008} to the list of methods. Counterfactual reasoning involves considering alternate outcomes of events, and the Socratic method can be used to guide discussions on this topic by encouraging critical thinking and self-reflection.
\end{comment}

\subsection{Illustrative Critical Reading Example}

To illustrate how these methods can practically be applied, let's use the example of critical reading. Critical reading is a crucial component of critical thinking, which involves evaluating the quality and credibility of written materials, from research papers to blog posts \cite{lai-etal-2017-race,PaulBinkerCT1990}. It requires a systematic and analytical approach, asking relevant questions, and using effective prompts to gain deeper understanding of the text \cite{Elder2010}.

\begin{table}[ht!]
%\vspace{-.1in}
\begin{center}
\begin{tikzpicture}
\node (table) [inner sep=0pt] {
\begin{tabular}{|p{0.56cm}|p{6.9cm}|}
\toprule
\textbf{} & \textbf{Function $\Gamma$ = CRIT($d$)} \\
\midrule
%& Function $\Gamma$ = CRIT($d$); \\
& \textbf{Input}. $d$: document; \textbf{Output}. $\Gamma$: validation score; \\
& \textbf{Vars}. $\Omega$: claim; $R$ \& $R'$: reason \& counter reason set; \\
& \textbf{Subroutines}. $Claim$(), $FindDoc$(), $Validate$(); \\
& \textbf{Begin} \\
\#1 & {\hspace{.2cm}}Identify in $d$ the claim statement $\Omega$; \\
\#2 & {\hspace{.2cm}}Find a set of supporting reasons $R$ to $\Omega$; \\
\#3 & {\hspace{.2cm}}For $r \in R$ eval $r \Rightarrow \Omega$ \\
& {\hspace{.5cm}}{If} $Claim$($r$), ($\gamma_r$, $\theta_r$) = CRIT($FindDoc$($r$)); \\
& {\hspace{.5cm}}{else}, ($\gamma_r$, $\theta_r$) = $V$($r \Rightarrow \Omega$); \\
%\#4 & {\hspace{.2cm}}Assessing rival arguments: \\
\#4 & {\hspace{.2cm}}Find a set of rival reasons $R'$ to $\Omega$; \\
\#5 & {\hspace{.2cm}}For $r' \in R'$, ($\gamma_{r'}$, $\theta_{r'}$) = V($r' \Rightarrow \Omega$) eval rival arguments; \\
\#6 & {\hspace{.2cm}}Compute weighted sum $\Gamma$, with $\gamma_r$, $\theta_r$, $\gamma_{r'}$, $\theta_{r'}$. \\
\#7 & {\hspace{.2cm}}Analyze the arguments to arrive at the $\Gamma$ score. \\
\#8 & {\hspace{.2cm}}Reflect on and synthesize CRIT in other contexts. \\
& \textbf{End} \\
\bottomrule
\end{tabular}
};
\draw [rounded corners=.5em] (table.north west) rectangle (table.south east);
\end{tikzpicture}
\end{center}
\caption{CRIT Pseudo-code \cite{CRITExtended2023}. (The symbol $\Rightarrow$ denotes both inductive and deductive reasoning.)}
\label{tab:CRIT}
%\vspace{-.2in}
\end{table}

\begin{comment}
\begin{table}[ht!]
%\vspace{-.1in}
\begin{center}
\begin{tikzpicture}
\node (table) [inner sep=0pt] {
\begin{tabular}{|p{0.56cm}|p{6.9cm}|}
\toprule
\textbf{} & \textbf{Function $\Gamma$ = CRIT($d$)} \\
\midrule
%& Function $\Gamma$ = CRIT($d$); \\
& Subroutines: $Claim$(), $FindDoc$(), $V$(); \\
\#1 & Identifying in $d$ the claim statement $\Omega$; \\
\#2 & Finding a set of supporting reasons $R$ to $\Omega$; \\
\#3 & For $r \in R$ \\
& ~~~~{If} $Claim$($r$), ($\gamma_r$, $\theta_r$) = CRIT($FindDoc$($r$)); \\
& ~~~~{else}, ($\gamma_r$, $\theta_r$) = $V$($r \Rightarrow \Omega$); \\
\#4 & Assessing rival arguments. \\
& ~~~~For $r' \in R'$ ($\gamma_{r'}$, $\theta_{r'}$) = V($r' \Rightarrow \Omega$); \\
\#5 & Computing a weighted sum score $\Gamma$, based on the strengths of both supporting and rival arguments. \\
\#6 & Analyzing the arguments to arrive at the $\Gamma$ score. \\
\#7 & Reflecting on and synthesizing the CRIT process in a different context, such as comparing perspectives from different time periods, personal opinions, or cultural settings. \\
\bottomrule
\end{tabular}
};
\draw [rounded corners=.5em] (table.north west) rectangle (table.south east);
\end{tikzpicture}
\end{center}
\caption{CRIT Pseudo-code. Input $d$ document, output $\Gamma$ validation score, V() validation routine, $\Omega$ conclusion, $R$ reason set, $R'$ rival reason set, ($\gamma_{r}$, $\theta_{r}$) validity and credibility scores of $r \Rightarrow \Omega$.}
\label{tab:CRIT}
%\vspace{-.2in}
\end{table}
\end{comment}

To aid in critical reading, we introduce a template called CRIT \cite{CRITExtended2023}, which stands for Critical Reading Inquisitive Template\footnote{It is important to note that the CRIT template presented here is intended for analyzing research, opinion, and news articles, and is not suitable for analyzing literature such as novels, prose, or poetry. Each type of literary work has its unique style and nature, which require tailored prompts to facilitate effective analysis.}. Given a document $d$, CRIT evaluates it and produces a validation score $\Gamma$. Let $\Omega$ denote the conclusion or claim of $d$, and let $R$ be the set of reasons supporting the claim. We define ($\gamma_r, \theta_r$) = V($r \Rightarrow \Omega$) as the causal validation function, where $\gamma_r$ denotes the validation score, $\theta_r$ the source credibility score,  for each reason-to-conclusion argument $r \Rightarrow \Omega$. Table~\ref{tab:CRIT} presents the pseudo-code of $\Gamma$ = CRIT($d$), which generates the final validation score $\Gamma$ for document $d$ with justifications.

In the following subsections, we will discuss how CRIT uses these five methods: 1) definition, 2) elenchus, 3) dialectic, 4) maieutics, and 5) counterfactual thinking.


\subsection{Method of Definition}

As shown in the pseudocode in Table~\ref{tab:CRIT}, 
the CRIT algorithm starts in
its step $\#1$, asking GPT-3 to identify the conclusion of a document. To avoid any misunderstandings, the prompt includes a clear instruction and definition. (In the square brackets, symbol {\em in} denotes a input slot to an LLM and {\em out} the output slot.)

\begin{table}[ht!]
\small
\begin{tabular}{p{0.6cm}|p{7.2cm}}
p1.1 & ``What is the conclusion in document [in: $d$] 
  [out: $\Omega$]? \\ 
& The conclusion statement may 
  be written in the last paragraph, near 
  keywords "in conclusion," "in summary," or "therefore."'' \\
\end{tabular}
\end{table}

We can use
the {\em definition} method to 
improve the understanding of the document. 
One approach is paraphrasing the prompt 
into multiple prompts and grouping them into an ensemble, similar to forming a thesis committee. (Section~\ref{sec:template} presents
prompt ensemble in details.)
Different members can phrase the same question in different ways or ask it from a different perspective.  For example:

\begin{table}[h!]
\small
\begin{tabular}{p{0.6cm}|p{7.2cm}}
p1.2 &  ``What is the issue addressed by [in: $d$] 
  [out: $\Omega$]?'' \\
p1.3 & ``What is the most important outcome presented in text [in: $d$]? [out: $\Omega$]''
\end{tabular}
\end{table}

Step $\#2$ in Table~\ref{tab:CRIT} prompts GPT-3 to find a set of supporting reasons. To further enhance the accuracy and comprehensiveness of the results, the prompt can ask for not only ``reasons'' but also ``theories,''``evidences,'' or ``opinions'' to query for the document's support to its conclusion, similar to the ensemble method.

\begin{table}[ht!]
\small
\begin{tabular}{p{0.6cm}|p{7.2cm}}
p2 & ``What are the supporting reasons [out: $R$] of conclusion \\
& [in: $\Omega$] of [in: $d$]? A reason can be a theory evidence or opinion.'' 
\end{tabular}
\end{table}

\begin{comment}
Note that prompts can be submitted all together or
one-by-one to GPT-3. Our empirical study 
on reading comprehension
samples~\cite{501Q2004} shows that issuing prompts one-by-one
generates output with finer details.  This is because
GPT-3 has a chance to examine a document multiple times
for slightly different purposes.
For teaching K-12 students critical reading, 
the one-by-one prompting is
better because it allows students to interact with
CRIT step-by-step.  
\end{comment}

\subsection{Method of Elenchus}

The method of elenchus is rooted in the Greek word ``elenchein,'' which translates to examine. This method involves cross-examining the results generated by GPT-3 to evaluate the consistency and coherence of the arguments. The goal is to arrive at a deeper understanding of the validity of the reasons and conclusion, and to identify any potential weaknesses or flaws in the arguments.

Step $\#3$ of the CRIT algorithm prompts GPT-3 to assess the validity of each reason $r \in R$ as justification for the conclusion $\Omega$ through the function V($r \Rightarrow \Omega$). To validate the reason-to-conclusion argument, CRIT must evaluate the presented reason and its causal relationship with the conclusion and conduct cross examination, which is precisely the task of the method of elenchus.

CRIT issues four prompts in step $\#3$ to evaluate the logic validity and source credibility of the $r \Rightarrow \Omega$ reasoning. CRIT first elicits supporting evidence for reason $r \in R$. This evidence can be a theory, an opinion, statistics, or a claim obtained from other sources. If the reason itself is a claim, then the sources that the claim is based on are recursively examined. The strength of the argument and its source credibility are rated on a scale of $1$ to $10$, with $10$ being the strongest.


\begin{table}[h!]
\small
\begin{tabular}{p{0.6cm}|p{7.2cm}}
p3.1 & ``What is the evidence for reason [in: $r$] to support
conclusion [in: $\Omega$] in document [in: $d$]? [out: evidence]'' \\ 
p3.2 & ``What is the type of evidence? A) a theory, B) an opinion, C) statistics, or {\color{red}D}) a claim from other sources?'' \\
p3.3 & ``If the evidence of reason [in: $r$] is {\color{red}D}),
  call CRIT recursively'' \\
p3.4 & ``How strongly does reason [in: $r$] support
  [in: $\Omega$] in document [in: $d$]? Rate argument validity [out: $\gamma_r$] and source credibility [out: $\theta_r$] between $1$ and $10$ (strongest).''
\end{tabular}
\end{table}

It may be beneficial to also incorporate the counter-argument method in order to gain a more comprehensive and balanced evaluation of the argument. This can result in a deeper understanding of the topic being discussed. We will be discussing this further in the next section.

\begin{comment}
\begin{table}[h!]
\small
\begin{tabular}{p{0.6cm}|p{7.2cm}}
\end{tabular}
\end{table}
\end{comment}

\subsection{Method of Dialectic}

The easiest way to mislead without lying outright is to leave out critical counterarguments from the reader.
CRIT relies on GPT-3 to generate and
evaluate counter arguments, similar to
how it prompts GPT-3 to extract and 
evaluate reasons. 

CRIT in its step $\#4$ asks GPT-3 to provide missing
rival reasons, and then pair rival reasons
with the conclusion to conduct validation.
There are two strategies to 
bring counter arguments to the surface.
The first strategy attacks the weakest 
arguments with the lowest scores and asking
GPT-3 to attack those arguments.

\begin{table}[h!]
\small
\begin{tabular}{p{0.6cm}|p{7.2cm}}
p4 & ``Is there a counterargument against [in: $r \Rightarrow \Omega$]? If so, provide counter reasons [output $R'$].'' \\
p5 & Similar to p3, except for replacing argument $r$ with rival argument $r'$.
\end{tabular}
\end{table}

For finding omitted information, CRIT can
query GPT-3 without quoting any $r \in R$,
and follow the same process. 
%At the end, CRIT can append to the $\gamma$ score with a $-\gamma$ score, and provide an alert to the reader with a summary of the counter argument. 

Next, in step $\#6$, CRIT computes an aggregated score by performing a weighted sum on the validation multiplied by the credibility scores of both arguments and counterarguments, and then outputs the final assessment score $\Gamma$.


\begin{table}[h!]
\small
\begin{tabular}{p{0.6cm}|p{7.2cm}}
p6 & ``Final score [out: $\Gamma$]. $\Gamma = 
\sum_{r \in R \cup R'} \gamma_r \times \theta_r / |R \cup R'|$.
\end{tabular}
\end{table}
%\noindent
%\subsubsection*{Remarks on Critical Reading vs. Thinking} 
%\hfill \break

\subsection{Method of Maieutics}
\label{sec:Maieutics}

The maieutic method derives from the Greek word ``maieutikos,'' meaning midwife. It is founded on the belief that a teacher's role is to facilitate students in bringing forth their own understanding of a subject, rather than simply conveying knowledge. Unlike the elenctic method, which aims to detect and eliminate false hypotheses, maieutics centers on helping students reveal their own understanding of a subject. In this dialogical method, the teacher asks questions that are intended to guide the student in discovering their own comprehension, rather than providing them with information or answers.

Continuing with GRIT, once the text has been scored in step $\#6$, it can be valuable for readers or students to enhance their analytical and writing skills by summarizing and analyzing the justifications produced by GPT-3. CRIT in its step $\#7$ can prompt GPT-3 to generate a report, which readers and students can then compare with their own notes.

\begin{table}[h!]
\small
\begin{tabular}{p{0.6cm}|p{7.2cm}}
p7 & ``For every $r \in R \cup R'$ justify the validity score $\gamma_r$ and source credibility score $\theta_r$ for argument $r \Rightarrow \Omega$.''
\end{tabular}
\end{table}

\subsection{Counterfactual Reasoning}
\label{sec:cf}

Counterfactual reasoning~\cite{WinArgument2006,Cross-Examination2021} can be seen as a natural extension of the Socratic method, as both involve questioning assumptions and exploring alternative perspectives. 
Counterfactual thinking involves imagining alternative scenarios to what actually happened, often using phrases like ``what if'' or ``if only.''
By incorporating counterfactual reasoning into prompt engineering, one can facilitate exploration of alternative possibilities and promote more nuanced and complex understanding of a given topic.

The final step of GRIT involves using the counterfactual method to encourage students to reconsider the arguments and counterarguments presented in the text based on new contextual information. CRIT can prompt students with questions such as ``what if the debate in the text took place now instead of in the 1950s?'' or ``what if the main event in the text occurred in Asia instead of in Europe?'' Students can express their own opinions and findings based on further reading and statistics, and challenge the conclusions drawn in the text. 

\begin{table}[h!]
\small
\begin{tabular}{p{0.6cm}|p{7.2cm}}
p8 & ``For every $r \in R \cup R'$, evaluate $r \Rightarrow \Omega$
in [in context].''
\end{tabular}
\end{table}


\subsection{Remarks on the Socratic Method and CRIT}

As we have shown that for critical reading,
GRIT uses three methods, definition, elenchus, and dialectic.  
For critical thinking, CRIT uses methods maieutics and counterfactual reasoning. For more explorative 
thinking, methods such as induction can be used for informal brainstorming, hypothesis elimination for removing weak propositions, and generalization for deriving principles from examples.

Please note that prompts can be submitted to GPT-3 either all together or one-by-one. Our empirical study on reading comprehension samples~\cite{501Q2004} demonstrates that issuing prompts one-by-one results in outputs with finer details. This is because GPT-3 has the opportunity to analyze a document multiple times for slightly different purposes. For teaching critical reading to K-12 students, one-by-one prompting is preferred as it allows students to engage with CRIT step-by-step.  However, for answering multiple-choice
questions, both prompting all together and one-by-one receive 
similar scores. We will conduct large-scale study with
ablation tests to investigate if adding or
deleting prompts and using different submission methods
make marked differences.

\begin{comment}
\begin{small}
\begin{verbatim}
\end{verbatim}
\end{small}
\end{comment}



==> Table_Contentiousness.tex <==
\begin{table*}[t!]
\vspace{-.05in}
\centering
\begin{footnotesize}
%\begin{tabular}{|p{0.6cm}|p{4.6cm}|p{5.0cm}|p{4.6cm}|}
\begin{tabularx}{\textwidth}{|p{0.6cm}|X|X|X|}
\toprule
\textbf{C.L.} & \textbf{Tone} & \textbf{Emphasis} & \textbf{Language} \\
\hline \hline
$0.9$ & Highly confrontational; focused on raising strong ethical, scientific, and social objections. & Flagging risks and downsides; ethical quandaries, unintended consequences, and exacerbation of inequalities. & Definitive and polarizing, e.g., ``should NOT be allowed,'' ``unacceptable risks,'' ``inevitable disparities.'' \\
\hline
$0.7$ & Still confrontational but more open to potential benefits, albeit overshadowed by negatives. & Ack that some frameworks could make it safer or more equitable, while advising caution in its use. & Less polarizing; ``serious concerns remain,'' ``needs more scrutiny.'' \\
\hline
0.5 & Balanced; neither advocating strongly for nor against gene editing. & Equal weight on pros and cons; looking for a middle ground. & Neutral; ``should be carefully considered,'' ``both benefits and risks.'' \\
\hline
0.3 & More agreeable than confrontational, but maintaining reservations. & Supportive but cautious; focus on ensuring ethical and equitable use. & Positive but careful; ``transformative potential,'' ``impetus to ensure.'' \\
\hline
0.0 & Completely agreeable and supportive. & Fully focused on potential benefits; advocating for proactive adoption. & Very positive; ``groundbreaking advance,'' ``new era of possibilities.'' \\
\bottomrule
\end{tabularx}
\end{footnotesize}
\vspace{-.1in}
\caption{Changes in Arguments of GPT-4 at Different Contentiousness Levels.}
\label{tab:contentiousness}
\vspace{-.2in}
\end{table*}


==> WikiUsageChallenges.tex <==
\section{Related Work}
\label{sec:related}

This section reviews existing literature related to content quality and bias mitigation in digital platforms, setting the stage for the methodologies employed in our study. Wikipedia's criteria for a ``featured'' article \cite{WikiQualityMetrics} emphasize attributes such as well-written prose, verifiability, breadth, depth, neutrality, and stability—qualities our research aims to enhance, with a particular focus on neutrality to address systemic biases \cite{Hube2017BiasInWikipedia,WikipediaBiasStudyField}.

\subsection*{Bias in Digital Media}
\label{sec:bias_in_digital_media}

Biases in Wikipedia and news media, which span gender, race, ideology, and geography, compromise content quality. Studies like Wagner et al. \cite{Wagner2015ItsAM} highlight thematic biases in biographies, reflecting structural issues in content representation. News outlets, categorized by political leanings \cite{AllSidesBiasChart}, range from far left to far right, a classification that parallels our approach to categorizing news articles.

\subsection*{Advancements in Quality Improvement}
\label{sec:quality_improvement}

To meet the standards of ``featured'' articles, automated techniques focus on enhancing accuracy and neutrality \cite{Mo_s_2023}. The advent of LLMs has inspired heuristic-based prompting methods aimed at improving NLP reasoning \cite{ChainOfThought2022,yao2023tree,zhang2023cumulative,allaway2023penguins,jung2022maieutic,PromptSurvey2023,sclar2023minding}. These methods, however, grapple with the uncertainties of abductive reasoning \cite{FlachKakas2000AbductionInduction}, particularly challenging in open-domain scenarios where complex inference chains are common \cite{chen2023universal}.

\subsection*{Bias Detection and Mitigation Techniques}
\label{sec:biases_detection_mitigation}

Traditional bias detection methods often focus on sentence-level Neutral Point of View (NPOV) labeling, but are hampered by the quality and subtlety of biases \cite{aleksandrovamultilingual}. Recent strategies for reducing biases in LLMs involve pre-processing, model adjustments, and post-processing with feedback \cite{Ferrara_2023}, yet challenges in interpreting feedback and addressing residual biases persist. Demonstrated in Section~\ref{sec:exp1}, the subjectivity of annotators significantly influences label assignment, revealing the difficulty in maintaining noncontroversial labels across controversial articles.

SocraSynth, our proposed system, leverages structured dialogues among multiple LLMs to surface and mitigate biases, providing a dynamic and interpretable strategy detailed in the following sections.


\begin{comment}
    
%%%%%%  move to the limitation section in the end...

\subsection*{Remarks on Merits and Limitations}
\label{sec:remarks_merits_limitations}

Distinguishing our approach is the use of multiple LLMs for both content evaluation and generation, reducing the risk of inheriting single-model biases \cite{li2023large}. While LLMs facilitate in-depth semantic analysis, we must remain vigilant about the accuracy, comprehensiveness, and legal aspects of content creation. Ensuring the integrity and legal compliance of LLM contributions is paramount to maintaining Wikipedia's reliability as a trusted knowledge repository.
\end{comment}

\begin{comment}

In 2020, an analysis of Wikipedia's top-100 most frequented pages showed significant interest in categories such as \textit{People}, \textit{Politics and History}, \textit{Sports}, \textit{Technology and Online Platforms}, \textit{Entertainment and Arts}, and \textit{Research and Education} \cite{WikiStatics2023}. Monthly page-view statistics further illustrate Wikipedia's diverse usage spanning \textit{Research and Learning}, \textit{Curiosity and Exploration}, and \textit{Entertainment} \cite{WikiGreat2023}. Table~\ref{tab:page_stats} presents the top-ten visited pages in November 2023, highlighting the variety and frequency of content updates, such as the daily revisions in sports-related articles compared to the less frequent updates in historical content.

\begin{table}[ht]
\centering
\begin{footnotesize}
\begin{tabular}{|c|l|r|r|r|}
\toprule
\hline
\textbf{Rank} & \textbf{Page} & \textbf{Edits} & \textbf{Pageviews} \\ \hline
1 & 2023 Cricket World Cup & 532 & 14,148,770 \\ \hline
2 & Cricket World Cup & 199 & 13,917,748 \\ \hline
3 & YouTube & 29 &  6,468,789 \\ \hline
4 & 1234 & 3 &  4,676,115 \\ \hline
5 & Cleopatra & 4 &  4,672,320 \\ \hline
6 & Tiger 3 & 546 &  4,525,333 \\ \hline
7 & Pornhub & 13 & 4,192,495 \\ \hline
8 & Deaths in 2023 & 2,188  & 3,870,414 \\ \hline
9 & XNXX & 33 & 3,837,659 \\ \hline
10 & 2024 Men's World Cup & 447 &  3,749,162 \\ \hline
\bottomrule
\end{tabular}
\end{footnotesize}
\vspace{-.1in}
\caption{Top 10 Pages Statistics in November 2023}
\vspace{-.15in}
\label{tab:page_stats}
\end{table}
\end{comment}

\begin{comment}
\begin{figure}[th!]
\begin{center}
\includegraphics[width=0.97\linewidth]{QualityPI-Chart.jpeg}
\end{center}
\caption{Distribution from Top Quality High Importance ($1.2\%$) to Low Quality Low Importance ($91.6\%$). Notably, the blue segment ($4.8\%$) signifies high-importance pages in need of improvement.}
\label{fig:wiki-pichart}
\vspace{-.1in}
\end{figure}
\end{comment}

\begin{comment}
%Figure~\ref{fig:wiki-quality} illustrates the distribution of article quality against their importance \cite{WikiQualityImportance2023}, categorizing articles into six levels of quality, from FA' (featured article) and FL' (featured list) to lower tiers, indicating areas needing improvement.

%Wikipedia also employs an "importance" scale, subjectively assessed by editors, dividing topics into four tiers: Top', High', Mid', and Low'. The data highlights that 4.8\% of content, considered important, suffers from lower quality, marking them as priorities for enhancement.

\begin{figure}[t!]
\vspace{-.1in}
\begin{center}
\includegraphics[width=1.00\linewidth]{Quality_Importance_Matrix_snapshot.png}
\end{center}
\vspace{-.15in}
\caption{Matrix of Wikipedia Quality vs. Importance.}
\label{fig:wiki-quality}
\vspace{-.2in}
\end{figure}

\subsection{Biases Assessment}
\label{sec:wiki-biases}
\end{comment}


==> WikipediaMomentofTruth.tex <==
\section*{Appendix: Wikipedia Moment of Truth}

According to New York Time's recent 
podcast given by \cite{WikiTruth2023},
Wikipedia faces challenges.  

\subsection{The Rise of GPT-3 and Its Implications}

In early 2021, a Wikipedia editor, known as Barkeep49, peered into the future and saw the rise of GPT-3, a precursor to the new chatbots from OpenAI. This technology, although untrustworthy in its nascent stages, presented a potential threat to Wikipedia and its human editors.

\subsection{The Unreliability and Potential of AI}

Barkeep49's experiment with GPT-3 revealed its tendency to mix fictional elements into factual answers. Despite these shortcomings, the editor was convinced of AI's inevitable role in content creation. He speculated on a future where AI could displace Wikipedia, just as Wikipedia had supplanted traditional encyclopedias.

\subsection{The Wikipedia Model: Endurance and Adaptation}

As Wikipedia marked its 22nd anniversary, it remained a testament to the internet's utopian early days, emphasizing open collaboration and knowledge sharing. However, its role as a factual netting for the digital world faced new challenges with the advent of AI.

\subsubsection{The Paradigm Shift in Information Access}

Wikipedia's integration into search engines, virtual assistants, and now AI chatbots represents a paradigm shift. Its content, ingested into knowledge banks of various platforms, plays a critical role in shaping the AI landscape.

\subsection{The Ethical Dilemma and Future Directions}

The ethical implications of AI-driven platforms like SocraSynth, and their impact on platforms like Wikipedia, present a complex dilemma. This paper aims to explore these themes further, delving into the potential positive and negative impacts of such technological advancements.


